Simplicial SMOTE: Oversampling Solution to the Imbalanced Learning Problem

SMOTE (Synthetic Minority Oversampling Technique) is the established geometric approach to random oversampling to balance classes in the imbalanced learning problem, followed by many extensions. Its idea is to introduce synthetic data points of the minor class, with each new point being the convex combination of an existing data point and one of its k-nearest neighbors. In this paper, by viewing SMOTE as sampling from the edges of a geometric neighborhood graph and borrowing tools from the topological data analysis, we propose a novel technique, Simplicial SMOTE, that samples from the simplices of a geometric neighborhood simplicial complex. A new synthetic point is defined by the barycentric coordinates w.r.t. a simplex spanned by an arbitrary number of data points being sufficiently close rather than a pair. Such a replacement of the geometric data model results in better coverage of the underlying data distribution compared to existing geometric sampling methods and allows the generation of synthetic points of the minority class closer to the majority class on the decision boundary. We experimentally demonstrate that our Simplicial SMOTE outperforms several popular geometric sampling methods, including the original SMOTE. Moreover, we show that simplicial sampling can be easily integrated into existing SMOTE extensions. We generalize and evaluate simplicial extensions of the classic Borderline SMOTE, Safe-level SMOTE, and ADASYN algorithms, all of which outperform their graph-based counterparts.

==> algorithms/todo.tex <==
To address

Introduction and motivation
- improve motivation, state the research question more explicitly
- highlight the application of topological data analysis ideas for data augmentation (add filtration viewpoint!)
- imbalanced solutions taxonomy: sampling-based, weighting-based, margin-based
- geometric data augmentation for the imbalanced learning problem — augmenting the minor class(es) only, not augmenting the labels 
Details
- provide the assumptions on data’s distribution and the level of class imbalance
- provide the details on datasets selection (UCI and LIBSVM datasets, typically used for the testing imbalanced learning problem)
- say more on hyperparameters selection, provide best k and p for each dataset (actually provide graphs of k and p)
- state how Mixup is applied, in the description of SMOTE add that it oversamples only the minority class (general data augmentation algorithm applied for the imbalanced learning problem)
- ROS/SMOTE/Mixup in terms of filtration of a metric space
- state that is sampling is done from the maximal simplices of p-skeleton of a clique complex
    - details on subsampling cliques according to the uniform distribution
- provide a (round) graph of SMOTE vs S-SMOTE, B/SMOTE vs B/S-SMOTE, along with statistical significance tests (maybe with some other methods?)

Complexity and running time
- provide the running time to emphasize the method is practical (also try larger datasets)
- provide the running time dependence on data’s size and dimensionality
- provide space complexity

Dependencies on hyperparameters
- provide sensitivity on k and p for several datasets (and several classifiers)

Metrics
- say more on F1 and MCC are complementary and MCC is preferred than means of per-class accuracies or ROC AUC, state why

Statistical significance testing
- multiple testing via Friedman-Nemenyi (Conover) test, visualization w/ critical difference diagrams

Extensions
- say more on simplicial extensions, we provide the results on Borderline SMOTE only due to it is best or second-best for non-simplicial oversampling methods

Reproducibility
- provide the code on the method and experiment for reproducibility, experiment.py

Binary and multi-class oversampling
- state that we consider only the binary classification problem, as the method trivially can be applied to the multi-class case (imbalanced MNIST-10, CIFAR-10, TinyImageNet-200)
- maybe: additional datasets (imbalanced versions of MNIST, CIFAR-10)
    - problem w/ mixup — superpositioned images, SMOTE and S-SMOTE — better looking due to the locality

Theoretical guarantees (not yet)
- if possible, replace the synthetic data experiment with theoretical guarantees section or an experiment showing the closeness of synthetic points to real ones generatively or discriminatively (Buzun)

Motivation

Vicinal distribution (vicinal risk minimisation, VRM), replace empirical density w/ data augmented density, works better if the density estimator parameters are chosen right [Vapnik]
- super-local vs global inductive bias (random upsampling vs random interpolation — Mixup)
- local methods — local linearity assumption of the data manifold, SMOTE can be improved further:
    - as SMOTE samples from two local points, it’s not sampling the whole space, visible as generating linear artefacts even in 2D (Figure, several datasets)
    - augment not the minority class, but its subset on the decision boundary (as the Borderline variant)

Мотивация с точки зрения решении существующей проблемы
- точка ближе к границе, пример с 3D
- sample diversity

Main results:
- generalize SMOTE and its several extensions
- provide the results of evaluation the simplicial generalisations of SMOTE and the best-performing variant of Borderline SMOTE
- provide the taxonomy of the geometric oversampling methods, based on neighborhood size and relation arity (including random oversampling)

Connection to data augmentation methods:
- data augmentation, unsupervised — augmenting data, w/o class dependence
- imbalanced learning — augmenting the minor class(es) only, either
    - without using information about class labels
    - with using information about class labels

New figures

- critical difference diagrams for the results in the main text
    - state that Simplicial SMOTE is significantly better than SMOTE
    - state that Borderline Simplicial SMOTE is significantly better than Borderline SMOTE
- graph, metrics dependence on k and p for several (all?) datasets (appendix?)
- graph, time dependence on data size for letter_img (largest) dataset

Model selection and evaluation

Nested cross-validation (stratified, repeated) with 5-fold inner (5 repeats) and outer (2 repeats) cross-validation procedures. In the grid search F1 and MCC was used for refitting.





Introduction

- imbalanced learning problem definition, context, minor and major classes, classifier bias — decision boundary moves away from the majority class
- existing solutions to the imbalanced learning problem: specialized classifiers, reweighing, resampling, margin/decision boundary altering
- geometric resampling methods (random oversampling, mixup — rename, SMOTE), their commonality (geometric model of data), difference (locality)
- resampling replaces the original empirical distribution with a vicinal distribution, proven to improve the solution of the original ERM problem
    - different assumptions — no assumptions (duplicate points), global linearity (Mixup), local linearity (SMOTE)
    - generative, modeling duality
        - precision (sample quality) — how well it models (RO highest precision, Mixup lowest), how well it respects the data topology such as disconnectedness of the distribution and topological holes
            - how much model samples are within the data support?
        - recall (data coverage) — how well it covers the data distribution support,
            - how much data samples are within the model support?
    - discriminative — for the discriminative downstream tasks such as classification it is not necessary to model the whole minor class distribution, only its subset on the decision boundary (i.e. Borderline SMOTE)
- issues of existing geometric resampling methods:
    - low data coverage, due to low-dimensional geometric models, which leads to artefacts and samples points farther from the major class
    - low sample quality of global methods (for curved, topologically complex distributions) do not respect the topology of the data distribution, convex hull argument
        - local methods as well see no difference between a region that could be sampled and not (a topological hole)
- proposed solution — to increase the number of points to generate a synthetic point implement a high-dimensional geometric model of a data, i.e. a simplicial complex (a union of simplices — convex polytopes spanned by an arbitrary number of points being sufficiently close, contrary to SMOTE and Mixup — , which model data with a union of segments). In terms of locality SMOTE is local, Mixup is global.
    - balanced precision/quality, due to locality, respects the disconnectedness
    - increased recall/coverage, due to the local convexity assumption
        - moves the decision boundary closer to the majority class
        - imposes a difference between dense regions and topological holes, respect holes

A number of resampling methods are geometric by nature, having in common the reliance to a geometric model of data, i.e. introducing new points within a neighborhood of existing data points or by their interpolation. Geometric resampling methods differ in terms of a neighborhood size or locality. For random oversampling \cite{Batista2004} that simply duplicates the existing points, the neighborhood of each point includes only the point itself, while for the label-independent Mixup \cite{Zhang2018} that introduces new synthetic points as the convex combination of randomly selected pairs of points, the neighborhood of each point includes all points of its class. Synthetic Minority Oversampling Technique (SMOTE) \cite{Chawla2002} introduces new synthetic points as the convex combination of pairs consisting of a data point and its nearest neighbors, that way the neighborhood of each point includes points of its class being sufficiently close.

From the data modeling standpoint, geometric resampling replaces the original empirical distribution with a vicinal distribution, by replacing the original empirical distribution density with data augmented density, an approach proved to improve the solution of the original problem if the density estimator parameters are chosen right \cite{Chapelle2000}. Data models can be quantified by two dual metrics. First, sample quality (precision) is how well it models the data, answering a question “how much model samples are within the data support?”. Second, data coverage (recall) is how well the model covers the data, answering the question “how much data samples are within the model support?”. Moreover, for the imbalanced learning problem where the data resampling is followed by the discriminative downstream tasks such as classification it is not necessary to model the whole minor class distribution, modeling its subset on the decision boundary will be sufficient.

From this we can deduce the issues of existing geometric resampling methods. First, the low data coverage, due to low-dimensional geometric models which use single or pairs of points to generate synthetic ones, which leads to artefacts and samples points farther from the major class. Second, the low sample quality of global neighborhood methods for topologically and geometrically complex data distributions, as by modeling data globally by a convex hull they do not respect the topology (multiple connected components and topological holes) and local geometry (curved areas) of the data distribution. 


- precision, quality, fidelity (how realistic sample is?)
- recall, coverage, diversity (how well sample capture variations of data?)


Decision based on technical merit, originality, potential impact, quality of execution, quality of presentation, related work, reproducibility of results, and ethics.

We are encouraging the (optional) use of the “Artifacts Available” badge in ACM’s Digital Library. If you release any code, dataset, or similar artifact to accompany your paper, and host it in a publicly available, archival repository for research artifacts that provides a Document Object Identifier (DOI), you are welcome to apply for this badge.

Decision based on technical merit, originality, potential impact, quality of execution, quality of presentation, related work, reproducibility of results, and ethics.

==> figures/algorithms.tex <==
\begin{figure*}[ht!] % [htbp]

\label{figure:models}
%\includegraphics[width=\textwidth]{figures/algorithms.png}
\includegraphics[width=\textwidth]{figures/teaser.jpg}

\vspace{-0.5em}
\caption{Geometric oversampling algorithms: a) Random oversampling, , b) Mixup, c) SMOTE, d) Simplicial SMOTE. Data's graph or simplicial models in blue, selected edges or simplices to sample and sampled synthetic points in red. With no inductive assumptions on data, Random oversampling just duplicates existing points. Assuming that synthetic data points lie within a convex hull of existing points, global methods like Mixup do not respect the intrinsic properties of data such as clusters and holes. While SMOTE, being a local method, improves on this, it still models the data with a union of $1$-dimensional cells, unable to sample all of the data's support. Simplicial SMOTE, by modeling data with a union of higher-dimensional simplices, samples dense areas of data's support while avoiding sampling from topological holes.
}

\end{figure*}

==> figures/cd_svm_f1.tex <==
\begin{figure*}[h!] % [htbp]

%\vspace{-0.5em}
\centering
\includegraphics[width=0.9\textwidth]{figures/cd_svm_f1.png}

%\vspace{-1em}
\caption{Critical difference diagram for the SVM classifier with RBF kernel and F1 score.}
\label{cd_gb_f1}
\Description{Critical difference diagram for the SVM classifier with RBF kernel and F1 score.}
\end{figure*}

==> figures/figure4.tex <==
\begin{figure*}[t!]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{17cm}{0cm}}
\end{center}

%\vspace{-0.75em}

\caption{Generalization of SMOTE variants. a) Borderline SMOTE, b) Safe-level SMOTE, c) ADASYN.}
\end{figure*}

%\vspace{-0.5em}

==> figures/parameters.tex <==
\begin{figure}[h!] % [htbp]

%\vspace{-0.5em}

\centering
\includegraphics[width=7.5cm]{figures/parameters/ecoli.png}

\vspace{-1em}
\caption{Parameters, $p$ versus $k$.}

\end{figure}

==> sections/__new.tex <==
\onecolumn
\section*{New}

Some text here

\subsection*{Motivation}

Motivation goes here

We were motivated by the assumption that a geometric model represented by a simplicial complex is better than one of the graph, i.e. the data distribution is well-approximated by a union of simplices of a geometric neighborhood complex for some set of the neighborhood size parameter $k$ and and the maximal simplex dimension $p$. We also hypothesize that $p$ could be related to the intrinsic dimension of the data, and the neighborhood size depends on data’s local geometry.

As we state in the last two paragraphs of introduction, one could not fill the whole data manifold using samples from the edges of the neighborhood graph as edges are $1$-dimensional. By increasing the dimension of simplices we fill more space, ideally to match the simplex dimension to the local intrinsic dimension of data. For the graphic explanation see \url{https://anonymous.4open.science/r/simplical-smote/motivation.png}.

% precision-recall argument
Precision and recall. Informally, these correspond to the average sample quality and the coverage of the sample distribution, respectively. Precision denotes the fraction of generated images that are realistic, recall measures the fraction of the training data manifold covered by the generator \cite{Kynkaanniemi2019}.

Low recall i.e. insufficient coverage of the underlying manifold \cite{Kynkaanniemi2019}.

Low recall is the insufficient coverage of the real distribution by the model.
Low precision is the low sample quality produced by the model, i.e. off the real distribution.

Real distribution $P$, model distribution $Q$.

% geometric arguments

% manifold assumption

\subsection*{Parameter sensitivity}

We provide parameter sensitivity on the neighborhood size $k$ and maximum simplex dimension $p$. Additional graphs could be seen in the appendix. We conclude that there are peaks in optimal values of $k$ and $p$, whilst the peak is more prominent for the latter. That is, as the classification tasks mostly benefits from increasing the neighborhood size,  the optimal value of $p$ generally lies between its possible minimum and maximum values.
[GRAPHS]

% default values of p
If a practitioner does not have a time for an extensive grid search of hyperparameters she/he can try to use Simplicial SMOTE with the default value of maximal simplex dimension $p$, which considers the exact maximal simplices in the neighborhood graph, depending on neighborhood size $k$, i.e. not limiting their dimension. This in many cases leads to better performance than of SMOTE, yet we obtained the best results by searching for the optimal maximal simplex size. We also observed that simply raising a dimension of a maximal simplex to sample from an edge, as did in SMOTE, to a triangle often resulted in better quality metrics of the downstream tasks.

\subsection*{Running time}

We provide the running time of an experiment on 23 datasets, with the same pipeline as in the paper including scaler, oversampler and logistic regression as the classifier. We run $5$-fold cross-validation repeated $5$ times for the neighborhood size parameter k=10. The maximal simplex dimension $p$ was set to $3$. Different values of p does not affect computation time as we our current implementation of clique expansion algorithm uses the NetworkX’s Bron-Kerbosch algorithm to find all maximal simplices and then subdivide them (which is inexpensive compared to MCE) to the $p$-simplices according to maximal simplex dimension p. Computation was run on 2x Intel(R) Xeon(R) Gold 6248R CPU @ 3.00GHz system, with 48 cores and 96 threads total.

\begin{itemize}
    \item SMOTE, k=10 – 15.03 sec (0.65 sec per dataset on average),
    \item Simplicial SMOTE, k=10, p=3 – 20.79 sec (0.90 sec per dataset on average)
\end{itemize}

To conclude, the running time of a typical scenario to fit an oversampler and a linear classifier $25$ times is only $1.4$ times slower for the Simplicial SMOTE compared to the original SMOTE algorithm on the benchmark datasets from the imbalanced-learn package.

\subsection*{Assorted}

% assumptions on the level of class imbalance
We had no specific assumptions on the level of class imbalance (like most of the literature). Common sense argument is that the class imbalance should be at a level where an empirical sample of the minor class is representative for the minor class distribution.

% assuptions of data
We assumed that a geometric model represented by a simplicial complex is better than one of the graph, i.e. the data distribution is well-approximated by a union of simplices of a geometric neighborhood complex for some set of the neighborhood size parameter $k$ and and the maximal simplex dimension $p$. We also hypothesize that $p$ could be related to the intrinsic dimension of the data, and the neighborhood size depends on data’s local geometry.

% "geometric" sampling methods
For a simple distributions with a single connected component, convex hull is a simplest geometric model of a dataset, a new synthetic point is any point within a convex hull. Yet, the Mixup-like sampling samples only a subset of a convex hull, its geometric model is a union of 1-dimensional segments spanned by all possible pairs of datapoints.

Our assumptions of data which are same of SMOTE are that the data distribution is of complex shape and topology (multiple connected components, presence of holes). The additional assumption that we make that is the dataset is \emph{locally convex}, i.e. the local regions spanned by the arbitrary number of points being sufficiently close could be used for the synthetic data generation, contrary to SMOTE which geometric model is still a union of 1-dimensional segments spanned by the pairs of datapoints being sufficiently close.

% vicinal risk minimizarion standpoint
Data augmentation methods are often viewed from a vicinal distribution standpoint, where one replaces the original empirical distribution which a new vicinal one, which is hypothesized to better represent the true distribution, which is generally unknown \cite{Chapelle2000}.

Based on various assumptions of data one can propose a oversampling algorithm. Random oversampling can be seen as most conservative approach, as it does not assume one could do any better than duplicating existing datapoints.

Our algorithm assumption is local convexity, that is a new synthetic point being the convex combination of existing data points being sufficiently close, will belong to the true distribution support with high probability.

Our 

% data augmentation taxonomy

% connection/difference btw data augmentation and the imbalanced learning problem
We want to highlight the connection between general data augmentation methods and the imbalanced learning problem. While having similar principles, i.e. geometric interpolation some methods are mostly known for its data augmentation usage, like Mixup, while SMOTE is mostly knows as the oversampling approach for the imbalanced leaning problem. In data augmentation - the oversampling is made for the whole dataset, for all  classes in supervised/unsupervised way, i.e. the information about classes may be used (for example Mixup's label interpolation) or not. In the imbalanced learning problem -- the oversampling is made for the subset of datasets, the minor class(es), in supervised/unsupervised way, the information about classes may be used (Borderline SMOTE, ADASYN) or not (SMOTE).

% Mixup for the imbalanced learning problem
Mixup for the imbalanced learning problem \cite{Bellinger2020,Chou2020,Galdran2021,Peng2023,Wang2023}.

% methods taxonomy based on a filtration of a metric space
In topological data analysis there is a concept of filtration of a metric space, where given all pairwise distances we can view them as edges of a graph and add them one by one in increasing order. ROS and Mixup correspond to the extremes of the filtration, with ROS being the zero step and Mixup the last one. SMOTE corresponds to a graph somewhere in between of the filtration, and Simplicial SMOTE to the clique complex of that graph. Next, one decides from simplices of which dimension to sample: 0-simplices for ROS, 1-simplices for Mixup and SMOTE, 2-simplices and greater for Simplicial SMOTE.

% synthetic data, local vs global
The purpose of the artificial data experiment was to show the importance of local sampling to respect data’s geometry and topology, which makes SMOTE-based algorithms better than Mixup. In all four examples if the sampling is not local, the synthetic points of the minor class shown in red would either mix with the points of the major class or would result in completely different topology of the decision boundary like in the circle inside the circle example.

% multiclass scenario
Our method can be used to handle the multi-class scenario, by oversampling all classes except the major to match it in size. Yet, as most of the existing works on SMOTE and its variants, we considered only the binary case.

% running time
The clique expansion stage does not depend on data dimensionality; for the $k$-nearest neighbors graphs with the same edge density there would not be an impact on the running time of the algorithm.

% cross-validation
We used the nested cross-validation for hyperparameter search and model evaluation. The outer cross-validation with 4 repeats and 5 splits. The inner cross-validation with 10 repeats and 4 splits.

% grid search details
We used the grid search for $k$ with step $2$, and for $p$ with step $1$ within a range which was dataset-specific, depending on the number of data points and features.

% results, statistical significance testing
We considered multiple classifiers/multiple datasets significance testing using the Friedman test with Nemenyi (Conover) post-hoc analysis \cite{Demvsar2006}. We provide the critical difference diagrams for each results table and the tables of post-hoc test p-values in the Appendix. Note that both Simplicial SMOTE and Borderline Simplicial SMOTE outperformed significantly there base counterparts, i.e. SMOTE and Borderline SMOTE.TheMatthewscorrelationcoefficient(MCC),instead,isamorereliablestatisticalratewhichproducesahigh score only if the prediction obtained good results in all of the four confusion matrix categories (true positives, false negatives, true negatives, and false positives), proportionally both to the size of positive elements and the size of negative elements in the dataset.

% reproducibility
To increase the reproducibility of our research and its potential impact we made available our method implemented in Python, along with the main experiment code at the anonymized repository \url{https://anonymous.4open.science/r/simplical-smote/}. We plan to release the computationally optimized version of our method upon the paper acceptance.

% F1/MCC complementariness
We report F1 and Matthew's correlation coefficient scores, as the complementary pair of metrics. F1 score emphasizes the correct classification of the minor class, while MCC considers all elements of the contingency table. The former one is the metric of choice when one is interested most in the correct classification in the minority class over the majority one, as F1 score is independent from the number of samples correctly classified as negative (i.e. of the major class) \citep{Davis2006,Chicco2020}. The latter considers all cells of the contingency table. MCC was shown to be preferable over ROC AUC and geometric mean of minor/major accuracies due to 1) a high score only if the binary predictor was able to cor- rectly predict the majority of positive data instances and the majority of negative data instances \cite{Chicco2020,Chicco2023}.
The Matthew's correlation coefficient (MCC) generates a high score in its interval only if the classifier scored a high value for all the four basic rates of the confusion matrix: sensitivity, specificity, precision, and negative predictive value. A high MCC always corresponds to a high ROC AUC, and not vice versa \cite{Chicco2023}.

The Matthew's correlation coefficient (MCC) is a reliable statistical rate which produces a high score only if the prediction obtained good results in all of the four confusion matrix categories, proportionally both to the size of positive elements and the size of negative elements in the dataset \cite{Chicco2020}.

\clearpage
\input{tables/results_knn_f1}
\input{tables/results_knn_mcc}

\twocolumn

==> sections/_introduction.tex <==
\section{Introduction}

% WHAT'S NEW?

% imbalanced learning problem, its context
The imbalanced learning problem is the learning from data when the minority class is dominated by the majority one \citep{He2009}. Many problems in data mining and data analysis are inherently imbalanced in the areas like finance (fraud detection) \citep{Wang2019,jiang2023benchmarking}, marketing (churn prediction) \citep{Liu2018},  medicine (medical diagnosis) \citep{Han2019}, industry (predictive maintenance) \citep{Sridhar2021}, etc. Often, the rare minority class (a credit fraud, a canceled subscription, the presence of a disease, an equipment failure) is of much more interest than the common majority one. Class imbalance causes the bias of classifiers towards the majority class \citep{Wallace2011}, as the naive classifier assigning all data points to the majority class will achieve an accuracy equal to the majority class proportion.

% imbalanced learning problem, solution 
% + sampling-based, weighting-based, margin-based
There are several solutions to overcome this problem: 1) cost-sensitive learning using a class-weighted loss function \citep{Thai2010} or specialized classifier algorithms \citep{Krawczyk2016,esposito2021ghost}, 2) matching the class cardinalities by undersampling the majority class \citep{Hoyos2021}, which leads to loss of data, and alternatively 3) oversampling the minority class by introducing new synthetic data points of the minority class \citep{Santoso2017}.
% - combination of oversampling and upsampling
% - reweighting
% - margin-based



% upsampling
% + simplest upsampling - random oversampling
% + geometric upsampling - local vs global
% + connection to the data augmentation methods
Upsampling techniques include local ones, such as random oversampling \citep{Batista2004}, i.e., randomly duplicating the required number of the minority class instances and global ones, such as Mixup \citep{Zhang2018} (without labels interpolation), which introduces the new synthetic points as the random convex combinations of randomly selected pairs of the minority class instances. The established oversampling method, Synthetic Minority Oversampling Technique (SMOTE) \citep{Chawla2002} introduces the new synthetic points as the random convex combinations of pairs consisting of a point and its nearest neighbors. This could be seen as the sampling from the edges of the neighborhood graph.

% motivation
% - random is too local, mixup is global, smote is local, yet could be improved further by considering combination of more that two points

% To address this, we propose...
Neighborhood graphs model the data as the union of $1$-dimensional cells, spanned by pairs of points, which is insufficient to sample from high-dimensional spaces. For example, even for a $2$-dimensional dataset, one could not introduce samples from the entire convex hull spanned by data points using SMOTE. Instead, if we model the data with the union of cells whose dimension is equal to the feature space, for example, a union of $2$-dimensional triangles, which are simplices spanned by triples of points, we could sample it.

\input{figures/algorithms}

Therefore, we introduce the generalization of SMOTE, called Simplicial SMOTE, thus sampling from the higher-dimensional simplices of the clique complex of a neighborhood graph. That is, a position of a new point is defined by the barycentric coordinates concerning a simplex spanned by an arbitrary number of data points being sufficiently close, i.e., being in the $p$-ary proximity relation.

\subsection*{Our contribution}

\begin{itemize}
    \item we propose a novel simplicial extension to the SMOTE algorithm and its modifications, where the new points are sampled from the simplices of the geometric neighborhood simplicial complex,
    \item we demonstrated that the proposed simplicial extension is orthogonal to various modifications of the SMOTE method by introducing simplicial generalizations of several popular SMOTE variants such as Borderline SMOTE, Safe-level SMOTE, and ADASYN,
    \item we experimentally demonstrate the the proposed technique is characterized by significant increase in performance for various classifiers and datasets from the \texttt{imbalanced-learn} library.
    %\item we classified existing geometric oversampling approaches (random oversampling, SMOTE, Mixup) within the neighborhood size and the proximity relation arity axes and positioned Simplicial SMOTE with respect to them.
\end{itemize}

==> sections/_methods.tex <==
\section{Proposed approach}

% WHAT"S NEW?

Geometric sampling methods assume that a synthetic point combines (several) existing data point(s). When designing such algorithms, one should decide upon 1) a neighborhood size of each data point, ranging from a point itself to all points of the dataset, and 2) several points a synthetic point is a combination of. Neighborhood relations can describe the former, while the latter corresponds to the relation arity. While popular sampling methods like SMOTE model data with a graph, complete or local, based on the binary neighborhood relations, our choice is to model the data with a simplicial complex based on neighborhood relations of arity greater than $2$.

% neighborhood graph
Consider a complete graph $H_n$ with a vertex set $X \in \mathbb{R}^d$ of cardinality $n$. A \emph{neighborhood graph} $G = (X, E) \subseteq H_n$ is a subgraph of $H_n$ such that the edge set $E \subseteq {n \choose 2}$ is instantiated according to a relation $R$ defining a neighborhood of each point $\mathcal{N}(x) = \{ x' \mid xRx' \}$.

For example, let $X$ be endowed with a distance function $d: X \times X \rightarrow \mathbb{R}_+$. A (symmetrized) $k$-nearest neighbor relation $R^{k\mathrm{NN}}$ on $X$ defining a \emph{$k$-nearest neighbors neighborhood graph} parameterized by $k \in \mathbb{N} \setminus \{0\}$ is
%\resizebox{\columnwidth}{!}{
\begin{equation}
    R^{k\mathrm{NN}}(k) = \left\{\hspace{0.15em}(x, y)~\big\vert~d(x, y) \leq \textrm{min}_k d(x, z),~z \in X \hspace{0.15em}\right\},
\end{equation}
%}
where $\min_k(\cdot)$ denotes the $k$-th minimum, hence $\arg\min_k(x, z)$ is the $k$-th neighbor of $x$.

An $\varepsilon$-ball relation $R^{\varepsilon}$ on $X$ defining the \emph{$\varepsilon$-ball neighborhood graph} given a scale parameter $\varepsilon \in \mathbb{R}_{\geq 0}$ is
\begin{equation}
    R^{\varepsilon}(\varepsilon) = \left\{(x, y)~\big\vert~d(x, y) \leq \varepsilon \right\},
\end{equation}
meaning that balls $B_x(\varepsilon/2) \cap B_{x'}(\varepsilon/2) \neq \emptyset$ of radius $\varepsilon/2$ centered at $x$ and $x'$ intersect.

Given a binary relation $R$, a \emph{$p$-ary relation} $P$ of $R$ is defined as a subset $Y$ of $X$ of cardinality $p$ such that $Y \times Y \subseteq R$, that is, a set $Y$ iff $xRx'$ for any pair $(x, x') \in Y$. A \emph{maximal $p$-ary relation} $C$ of $R$ defined as a subset $Y$ of $X$ of cardinality $p$ that is maximal concerning inclusion \citep{Henry2011}.

Whether a binary neighborhood relation corresponds to an edge in a neighborhood graph, a $p$-ary relation corresponds to a graph's $(p+1)$-clique, more generally, a $p$-simplex in a neighborhood simplicial complex over the vertex set $X$. Points can belong to more than one simplex. All simplices containing a point $x$ are subsets of its neighborhood $\mathcal{N}(x)$ \citep{Henry2011}.

% Simplicial SMOTE
\subsection{Simplicial SMOTE}

% extend proximity relation to be general k-points

% barycentric coordinates w.r.t. simplex, i.e., its spanning points

We classified the existing approaches to geometric data modeling and sampling based on the neighborhood relation size and arity. We propose a simple yet effective generalization of SMOTE by considering a general $k$-ary proximity relation. That is, instead of binary relation leading to the proximity graphs, we believe the $k$-ary relation leads to proximity simplicial complex, resulting in the high-dimensional data model, contrary to a graph which is locally $1$-dimensional.

Given a set $X$, an \emph{(abstract) simplicial complex} $K$ is a collection of subsets of $X$ called \emph{simplices} such that if a simplex $\sigma$ is in $K$, then all of its subsets $\tau \subseteq \sigma$ are also in $K$. Let $\mathrm{\Lambda}_p$ be the set of all vectors of $p+1$ elements, such that $\lambda_i \geq 0$ and $\sum_{i=0}^k \lambda_i = 1$. Given a set of $p+1$ points $\{\mathbf{x}_i\}_{i=0}^p$ in an $d$-dimensional Euclidean space a \emph{geometric $p$-simplex} $\sigma$ is defined


\begin{equation}
    \sigma_{\mathbf{x}_0,\dots,\mathbf{x}_p} = \left\{ \sum_{i=0}^p \lambda_i \mathbf{x}_i \bigm\vert \boldsymbol{\lambda} \in \mathrm{\Lambda}_p \right\}.
\end{equation}

We call the elements of $\boldsymbol{\lambda}$ \emph{barycentric coordinates} w.r.t. the points spanning a simplex. Barycentric coordinates could be mapped into Euclidean coordinates, resulting in a synthetic point:
\begin{align}
    \hat{\mathbf{x}}_{\mathbf{x}_0,\dots,\mathbf{x}_p}(\boldsymbol{\lambda})
    &= \lambda_0\mathbf{x}_0 + \dots + \lambda_p\mathbf{x}_p\\
    %&= \begin{pmatrix} \lambda_0 \\ \vdots \\ \lambda_p \end{pmatrix}^T \mathbf{X}\\
    \nonumber &= \boldsymbol{\lambda}^T \mathbf{X}.
\end{align}

An example of a geometric complex is the \emph{Vietoris-Rips complex} parameterized by the scale parameter $\varepsilon \in \mathbb{R}_{\geq 0}$

\begin{equation}
    K^{VR}(\varepsilon) = \left\{ (x_0, \dots, x_p) \bigm\vert  d(x_i, x_j) \leq \varepsilon,~\forall i,j \right\}.
\end{equation}

More generally, with any graph, its clique complex could be associated by \emph{expansion}, that is, a complex $K(G)$ has the same vertices and edges $G$, and $(k+1)$-cliques of $G$ are simplices of $K(G)$. The Vietoris-Rips complex is the clique complex of an $\varepsilon$-ball neighborhood graph.

% k-skeleton
Simplicial complexes can be huge as they grow exponentially w.r.t. $p$, so one can work with its smaller subcomplexes. A \emph{$p$-skeleton} $L$ of a simplicial complex $K$ is the subcomplex of $K$ with the dimension of simplices at most $p$. Algorithmically, this corresponds to finding cliques up to dimension $p+1$ instead of maximal cliques.

\input{algorithms/algorithm1}

We outline the Simplicial SMOTE method in Algorithm 1. Note that it has only two hyperparameters, namely the neighborhood size ($k$ for kNN neighborhood graph) and the maximal arity of neighborhood relation (with $p=\mathtt{"maximal"}$ by default).

% taxonomy
\subsection{Taxonomy of geometric sampling methods}

To provide the better understanding of the positioning of the proposed Simplicial SMOTE method among we give the taxonomy of geometric sampling methods (Fig.~\ref{figure:teaser}) based on the neighborhood and the arity of the neighborhood relation, summarizing them in Table \ref{table:classification}.

\input{tables/taxonomy}

%\subsubsection*{Random}

% tolerance
% For random oversampling, the proximity relation is $xRx,~\forall x$, i.e. the point is only relates to itself. With the pre-class cardinality equal to $1$, synthetic points are duplicates of existing ones.

% neighborhood, cells
For random oversampling, a neighborhood of each point is only the point itself, resulting in synthetic points being duplicates of existing data points.

%\subsubsection*{Mixup}

% For Mixup, the proximity relation is $xRx',~\forall (x, x')$, i.e. all points are related to each other.

For global sampling, a neighborhood of each point is global, resulting in the complete graph as the data model, with synthetic points as convex combinations of pairs of data points sampled from the edges of the complete graph.

%\subsubsection*{SMOTE}

For SMOTE, a neighborhood of each point is local, defined via a kNN or $\varepsilon$-ball neighborhood relation, resulting in a neighborhood subgraph of the complete graph as the data model. Synthetic points are convex combinations of pairs of data points from the neighborhood graph edges.

%\vspace{-0.75em}
%\begin{align}
%    \hat{\mathbf{x}}_{\mathbf{x}_0,\mathbf{x}_1}(\alpha)
%    &= \alpha \mathbf{x}_0 + (1 - \alpha) \mathbf{x}_1.
%\end{align}

\input{figures/synthetic}

% generalizations
\subsection{Simplicial generalizations of SMOTE variants}

%\input{figures/generalizations}

% \begin{equation}
%     \nabla(\mathbf{x}, \mathbf{x}') = \frac{\mathrm{\Delta}^+_\mathbf{x}}{\mathrm{\Delta}^+_\mathbf{x'}} = \frac{k^+_\mathbf{x}}{k_\mathbf{x}} \frac{k_\mathbf{x'}}{k^+_\mathbf{x'}}.
% \end{equation}

% dataset, minority, and majority classes
Consider a dataset $\mathcal{X} = \{ \mathbf{x}_i, y_i \}_{i \in 1, \dots, n}$, where $\mathbf{x}_i \in \mathbb{R}^n$ and $y_i \in \{0, 1\}$. By convention, we denote the \emph{minority class} $\mathcal{X}^+ = \{ \mathbf{x}_i \mid y_i = 1 \}_{i \in 1, \dots, n^+}$ as positive, and the \emph{majority class} $\mathcal{X}^- = \{ \mathbf{x}_j \mid y_i = 0 \}_{i \in 1, \dots, n^-}$ as negative of sizes $n^+ < n^-$ respectively, with $n = n^+ < n^-$.

% minority and majority neighborhoods
We denote the \emph{minority neighborhood} of $\mathbf{x}_i$ are the points of the minority class within a given neighborhood of a point $\mathcal{N}^+(\mathbf{x}_i) = \{ \mathbf{x}_j \mid \mathbf{x}_i \sim \mathbf{x}_j, y_j = 1 \}_{j \in 1, \dots, k^+}$, and the \emph{majority neighborhood} of $\mathbf{x}_i$ as $\mathcal{N}^-(\mathbf{x}_i) = \{ \mathbf{x}_j \mid \mathbf{x}_i \sim \mathbf{x}_j, y_j = 0 \}_{j \in 1, \dots, k^-}$ of sizes $k^+$ and $k^-$ respectively. The majority and minority points ratios within a given neighborhood are defined as $\mathrm{\Delta^+}(\mathbf{x}_i) = k^+/k$ and $\mathrm{\Delta^-}(\mathbf{x}_i) = k^-/k$ respectively. Given two points from a majority class $\mathbf{x}, \mathbf{x}'$, the \emph{safe-level ratio} is defined $\nabla(\mathbf{x}, \mathbf{x}') = \frac{\mathrm{\Delta^+}(\mathbf{x})}{\mathrm{\Delta^+}(\mathbf{x'})}$.

The original SMOTE algorithm constructs the minority neighborhood graph and samples points from its edges without considering the majority class. Several variants of the SMOTE algorithm improve reinforcing the points close to the boundary between types by considering the density of the majority class relative to the points from the minority.

\begin{itemize}
    \item Borderline SMOTE \cite{Han2005} hard modifies the minority neighborhood graph, setting zero probability to sample synthetic points based on only points outside the borderline subset (i.e., the union of safe and noise points). The probability of sample points from simplices spanned by borderline and borderline and outside points remains the same.
    \item ADASYN \cite{He2008} hard/soft modifies the minority neighborhood graph, zeroing/lowering probabilities to sample synthetic points using points in the safe region. The probability of sample points from simplices changes proportionally to their safety/homogeneity ratio (the higher the homogeneity -- the lower the probability).
    \item Safe-level SMOTE \cite{Bunkhumpornpat2009} leaves the minority neighborhood graph intact but modifies the barycentric coordinate weights on simplices, adding more weight to sample synthetic points using points with a higher safety/homogeneity ratio.
\end{itemize}

We generalize the SMOTE algorithm variants to use the simplicial sampling scheme.

\subsubsection{Simplicial Borderline SMOTE}

The extension assumption is that the examples on the borderline and the ones nearby are more apt to be misclassified than the ones far from the borderline and, thus, more important for classification. The examples far from the borderline may contribute little to classification results.

The \emph{borderline subset} of the minority class $B(\mathcal{X}^+)$ is defined

% borderline subset
\begin{equation}
    B(\mathcal{X}^+) = \left\{ \mathbf{x}_i, y_i = 0 \bigm\vert \frac{|\mathcal{N}^+(\mathbf{x}_i)|}{|\mathcal{N}(\mathbf{x}_i)|} < 1/2, |\mathcal{N}^+(\mathbf{x}_i)| \neq 0 \right\}
\end{equation}
that is the points whose the larger part of the nearest neighbors belong to the majority class, except those whose nearest neighbors are completely majority class instances and are considered noise. The new points are the convex combination of the simplices of a simplicial complex built upon the borderline points and their nearest neighbors from the minority class.

\subsubsection{Simplicial Safe-level SMOTE}

The original SMOTE algorithm considers sampling from a $k$-simplex according to the Dirichlet distribution $\mathrm{Dir}(\boldsymbol{\alpha})$, where $\boldsymbol{\alpha} \in \mathbb{R}_{> 0}^k$. Without any further assumptions, the distribution is symmetric, i.e., all of the vector $\boldsymbol{\alpha}$ elements have the same value (usually $1$, resulting in the uniform distribution on a simplex). Safe-level SMOTE modifies the elements of $\boldsymbol{\alpha}$ by setting them based on the ratio of majority neighborhood ratios, resulting in synthetic points to be generated closer to safer minority points, i.e., having a larger proportion of neighbors of the same class. A simplicial generalization is to set the parameter $\alpha_i = 1 + \Delta^+(x_i)$.

\subsubsection{Simplicial ADASYN}

While Borderline SMOTE answers the question from which simplex to sample, selecting simplices spanned by borderline points, and Safe-level SMOTE answers the question from where precisely on a simplex to sample sampling closer to safer points, ADASYN answers the question of how much to sample from a simplex, inversely proportional to the average safety of points. Therefore, its simplicial generalization is to average arbitrary safety values instead of just a pair.

Borderline Simplicial SMOTE benefited most from the proposed sampling scheme, showing increased performance relative to both original SMOTE and Borderline SMOTE.

\input{tables/results_synthetic_f1}

% complexity analysis
\subsection{Complexity analysis} % shorten!

Algorithm complexity depends on complexity of the neighborhood graph construction and expansion. The naive nearest neighbor search have complexity of $O(n^2)$, while approximated nearest neighbor search lowers it to $O(n)$.

Enumerating all maximal cliques in a graph with $n$ vertices and $m$ edges is an NP-complete problem, requiring exponential time in the worst case. Up to $n^{n/3}$ maximal cliques exist in a graph with $n$ vertices \citep{Moon1965}. Yet, as the neighborhood graphs are sparse, the various bounds were given regarding the number of edges, node degree, and arboricity of a graph. In a graph with maximum degree $\delta$ the time complexity of maximal clique enumeration (MCE) is $O(\delta^4)$ per clique and $O((n - \delta)3^{\delta/3}\delta^4)$ total \citep{Makino2004,Eppstein2013}. The \emph{arboricity} is the minimum number of edge-disjoint spanning forests into which the graph can be decomposed. For a graph of arboricity $a$, the complexity of MCE is $O(am)$ \citep{Chiba1985}.

%Graph expansion could also be done via maximal clique enumeration (MCE). It is shown that the time complexity of MCE is $O(m)$, thus linear in the number of edges \citep{Yu2017,Yu2019}.

Enumeration of all cliques up to the size $p$ can be done in either inductive, incremental, or top-down enumeration approach after solving the MCE problem \citep{Zomorodian2010}. Recently, an algorithm conjectured to be optimal was proposed for this task, which is on average was shown to be approximately a magnitude faster than the incremental algorithm in practice \cite{Rieser2023}.

==> sections/_related.tex <==
%\newpage
\section{Related work}

% WHAT'S NEW?
% - ?
% - ?
% - ?

% SMOTE
% sampling generalizations

% SMOTE extensions
% - borderline/SVM SMOTE, safe-level, ADASYN, k-Means SMOTE, etc.

% borderline SMOTE
% - minority class density (ck-NN \citep{Berry2019}, LDAS \citep{Yan2022})
% - relative minority/majority class densities (safe-level, ADASYN)
% - decision manifold instead of minority class manifold (borderline, SVM)
% - dimensionality reduction (PCA SMOTE, Delaunay, DeepSMOTE)
% - sampling (k-means, hierarchical clustering, shortest paths, Delaunay?)
% - proximity graphs (Gabriel graph, relative neighbor graph, ...)

% decision manifold
The original SMOTE algorithm introduces synthetic points from the geometric model of the minority class manifold. Several variants of SMOTE instead propose to sample synthetic points from the minority class part of the decision manifold, i.e., the minority points lying on the boundary between classes. The decision manifold is estimated in several ways; Borderline SMOTE \citep{Han2005} estimates the decision manifold by taking the minority class local density around each minority data point, while SVM SMOTE \citep{Nguyen2011} first takes the points corresponding to the support vectors of the SVM classifier.

In Safe-level SMOTE \citep{Bunkhumpornpat2009}, a value called safe level ratio is assigned to each edge of the neighborhood graph built over minority class instances, which is the ratio of the numbers of minority class instances for a point $x$ and its neighbor $x'$. If the number of the minority class instances in the neighborhoods of $x$ and $x'$ are zero, no synthetic examples are generated from that edge. Otherwise, a new synthetic sample is a convex combination of the points, and the coefficient depends on the ratio, being close to the minority example with more neighbors of the minority class.

In ADASYN \citep{He2008}, for each minority point, a ratio of majority examples in the neighborhood is computed. The new points are the convex combination of minority class points, with the number of synthetic examples generated using a given minority example being inversely proportional to that ratio.

% clustering-based SMOTE variants
% Several SMOTE extension use clustering schemes for oversampling. MWMOTE \citep{Barua2012} first identifies the hard-to-learn informative minority class samples and then generates the synthetic samples from the weighted informative minority class samples using a clustering approach. In AHC \citep{Cohen2006}, the minority class is clustered using agglomerative hierarchical clustering, obtaining several clusters at different levels of resulting dendrograms. The new points are the centroids of the clusters, points in the interior of the polytopes spanned by an arbitrary number of points, with the distance less or equal to the chosen histogram level.

MWMOTE \citep{Barua2012} first identifies the hard-to-learn informative minority class samples and then generates the synthetic samples from the weighted informative minority class samples using a clustering approach. In Density-based SMOTE (DBSMOTE) \citep{Bunkhumpornpat2012}, minority class examples are partitioned into disjointed clusters by the DBSCAN algorithm \citep{Ester1996}. The new points are the random convex combinations of two points from the random edge of the shortest path connecting minority points with the pseudo-centroid point, which is the closest to the cluster centroid. LVQ-SMOTE \citep{Nakamura2013} oversamples the minority class, first approximating is using a set of prototype points obtained by LVQ (Learning Vector Quantization) algorithm \cite{DeVries2016}.

Mixup, a geometric method, introduces new synthetic points as a convex combination of a pair of existing points randomly chosen from a dataset \citep{Zhang2018}. Fitting parametric distributions to data, such as the Gaussian distribution, is also used for the minority class oversampling in the imbalanced data classification problem \citep{Xie2020}.

Our work improves the SMOTE modeling and sampling scheme by modeling data with a geometric simplicial complex \citep{Boissonnat2018,Dey2022}, which is the higher-dimensional generalization of a graph. Contrary to global methods such as Mixup or fitting Gaussian distribution, it respects local topological features of data such as clusters and topological holes. The new sampling scheme is orthogonal to most SMOTE improvements and could be used cooperatively with them. 

% density
% 

% relative density
% - 

% dimensionality reduction
% - PCA, autoencoder, Laplacian eigenmaps, random projections

% sampling
% - geometric SMOTE, HS-SMOTE (hyperspheres and hypercubes)
% - k-means SMOTE, AHC (clustering-based)
% - DBSMOTE (density ridges)

% our contribution -- sampling from simplices
% - k-ary sampling method, closure of the binary proximity relation
% - orthogonal to density, including relative minority/majority densities, borderline, dimensionality reduction extension

% \begin{itemize}
%     % decision manifold
%     \item Borderline SMOTE \citep{Han2005} hard modifies the minority neighborhood graph, setting zero probability to sample synthetic points based on only points outside the borderline subset (i.e., the union of safe and noise points). The probability of sample points from simplices spanned by borderline and borderline and outside points remains the same.
%     \item ADASYN \citep{He2008} hard/soft modifies the minority neighborhood graph, zeroing/lowering probabilities to sample synthetic points using points in the safe region. The probability of sample points from simplices changes proportionally to their safety/homogeneity ratio (the higher the homogeneity - the lower the probability).
%     \item Safe-level SMOTE \citep{Bunkhumpornpat2009} leave the minority neighborhood graph intact but modifies the barycentric coordinate weights on simplices, adding more weight to sample synthetic points using points with higher safety/homogeneity ratio.
% \end{itemize}

==> sections/methods_taxonomy.tex <==
% taxonomy
\subsection{Taxonomy of geometric sampling methods}

To provide the better understanding of the positioning of the proposed Simplicial SMOTE method among we give the taxonomy of geometric sampling methods (Fig.~\ref{figure:teaser}) based on the neighborhood and the arity of the neighborhood relation, summarizing them in Table \ref{table:classification}.

\input{tables/taxonomy}

%\subsubsection*{Random}

% tolerance
% For random oversampling, the proximity relation is $xRx,~\forall x$, i.e. the point is only relates to itself. With the pre-class cardinality equal to $1$, synthetic points are duplicates of existing ones.

% neighborhood, cells
For random oversampling, a neighborhood of each point is only the point itself, resulting in synthetic points being duplicates of existing data points.

%\subsubsection*{Mixup}

% For Mixup, the proximity relation is $xRx',~\forall (x, x')$, i.e. all points are related to each other.

For global sampling, a neighborhood of each point is global, resulting in the complete graph as the data model, with synthetic points as convex combinations of pairs of data points sampled from the edges of the complete graph.

%\subsubsection*{SMOTE}

For SMOTE, a neighborhood of each point is local, defined via a kNN or $\varepsilon$-ball neighborhood relation, resulting in a neighborhood subgraph of the complete graph as the data model. Synthetic points are convex combinations of pairs of data points from the neighborhood graph edges.

% \vspace{-0.75em}
% \begin{align}
%    \hat{\mathbf{x}}_{\mathbf{x}_0,\mathbf{x}_1}(\alpha)
%    &= \alpha \mathbf{x}_0 + (1 - \alpha) \mathbf{x}_1.
% \end{align}

==> sections/rebuttal.tex <==
\clearpage
\input{tables/results_lr_f1}

%\clearpage
\input{tables/results_dt_f1}

==> sections/rebuttal25.tex <==
\clearpage
\input{tables/results_lr_f1_25}
\input{tables/results_dt_f1_25}

%\clearpage
\input{tables/results_svm_linear_f1_25}


==> tables/_results_knn_f1.tex <==
\begin{table*}[h!]

\caption{Classification results on benchmark datasets for the $k$-NN classifier. F1 score averaged over $5$ repeats of $5$-fold (outer) cross-validation is reported. \textcolor{red}{\textbf{Best}} and \textcolor{blue}{\textbf{second-best}} results are highlighted. Results are \underline{underlined} when the Simplicial SMOTE and simplicial generalizations of Borderline SMOTE, Safe-level SMOTE and ADASYN methods are better or equal to SMOTE and the original versions, respectively.}
\label{table:knn_f1}

%\vspace{-0.5em}

\centering

%\renewcommand{\arraystretch}{1.2}

\resizebox{\textwidth}{!}{

\begin{tabular}{l|rrrrrrrrrr|rrrr}
\toprule
 & \textbf{Imbalanced} & \textbf{Random} & \textbf{Global} & \textbf{SMOTE} & \textbf{Border.} & \textbf{Safelevel} & \textbf{ADASYN} & \textbf{MWMOTE} & \textbf{DBSMOTE} & \textbf{LVQ} & \textbf{Simplicial} & \textbf{S-Border.} & \textbf{S-Safe.} & \textbf{S-ADASYN} \\  \midrule

ecoli           &     0.5780 &     0.5501 &     0.5864 &     0.5822 &     0.5853 &     \underline{0.5781} &     0.5705 &     0.5980 &     0.6336 &     0.5827 &     \underline{0.6275} &     \underline{0.6151} &     0.5688 &     \underline{0.6280} \\
optical\_digits &     0.9670 &     0.9491 &     0.9427 &     0.9415 &     \underline{0.9559} &     \underline{0.9439} &     \underline{0.9442} &     0.9376 &     0.9491 &     0.9618 &     \underline{0.9443} &     0.9557 &     0.9425 &     0.9423 \\
pen\_digits     &     0.9927 &     0.9906 &     0.9895 &     0.9906 &     0.9925 &     0.9900 &     \underline{0.9917} &     0.9907 &     0.9922 &     0.9928 &     \underline{0.9915} &     \underline{0.9925} &     \underline{0.9912} &     0.9911 \\
abalone         &     0.1808 &     0.3326 &     0.3842 &     0.3501 &     0.3586 &     \underline{0.3727} &     0.3448 &     0.3753 &     0.3281 &     0.3078 &     \underline{0.3698} &     \underline{0.3725} &     0.3614 &     \underline{0.3594} \\
sick\_euthyroid &     0.5565 &     0.5694 &     0.5872 &     0.5708 &     0.5684 &     0.5246 &     0.5650 &     0.5654 &     0.6081 &     0.5800 &     \underline{0.6049} &     \underline{0.5981} &     \underline{0.5962} &     \underline{0.6047} \\
spectrometer    &     0.7618 &     0.8493 &     0.8382 &     0.8430 &     \underline{0.8543} &     0.8274 &     0.8423 &     0.8551 &     0.7968 &     0.8209 &     \underline{0.8548} &     0.8485 &     \underline{0.8386} &     \underline{0.8465} \\
car\_eval\_34   &     0.6018 &     0.5830 &     0.5718 &     0.5774 &     0.5913 &     0.5886 &     0.5851 &     0.6490 &     0.5830 &     0.7165 &     \underline{0.6296} &     \underline{0.6081} &     \underline{0.6321} &     \underline{0.6341} \\
us\_crime       &     0.3676 &     0.4429 &     0.4404 &     0.4188 &     0.4567 &     \underline{0.4346} &     0.4144 &     0.4062 &     0.4429 &     0.4634 &     \underline{0.4313} &     \underline{0.4687} &     0.4210 &     \underline{0.4236} \\
yeast\_ml8      &     0.0375 &     0.1426 &     0.1613 &     0.1592 &     \underline{0.1659} &     0.1542 &     0.1578 &     0.1603 &     0.1426 &     0.1643 &     \underline{0.1598} &     0.1658 &     \underline{0.1601} &     \underline{0.1586} \\
scene           &     0.1004 &     0.2500 &     0.2499 &     \underline{0.2386} &     0.2471 &     \underline{0.2452} &     \underline{0.2309} &     0.2364 &     0.1101 &     0.2579 &     0.2251 &     \underline{0.2482} &     0.2219 &     0.2259 \\
libras\_move    &     0.6997 &     0.8031 &     0.7702 &     \underline{0.7672} &     \underline{0.7661} &     0.7362 &     0.7519 &     0.7874 &     0.8031 &     0.8029 &     0.7560 &     0.7568 &     \underline{0.7640} &     \underline{0.7525} \\
thyroid\_sick   &     0.4966 &     0.5239 &     0.5246 &     0.5255 &     0.5307 &     0.4620 &     0.5214 &     0.5245 &     0.5095 &     0.5031 &     \underline{0.5504} &     \underline{0.5459} &     \underline{0.5271} &     \underline{0.5579} \\
coil\_2000      &     0.0457 &     0.1745 &     0.1726 &     0.1709 &     \underline{0.1759} &     0.1677 &     0.1711 &     0.1748 &     0.0533 &     0.1168 &     \underline{0.1714} &     0.1748 &     \underline{0.1703} &     \underline{0.1743} \\
solar\_flare\_m0 &     0.0510 &     0.2192 &     0.2043 &     0.2077 &     0.2262 &     0.2280 &     \underline{0.2188} &     0.2120 &     0.0486 &     0.2126 &     \underline{0.2189} &     \underline{0.2337} &     \underline{0.2340} &     0.2171 \\
oil             &     0.3156 &     0.4467 &     0.4592 &     0.4428 &     0.4674 &     0.3784 &     0.4240 &     0.4191 &     0.4467 &     0.4626 &     \underline{0.5074} &    \underline{0.5062} &     \underline{0.4267} &     \underline{0.4777} \\
car\_eval\_4    &     0.1294 &     0.3815 &     0.4810 &     0.4443 &     0.4472 &     0.4121 &     0.4371 &     0.5240 &     0.3815 &     0.6771 &     \underline{0.5749} &     \underline{0.5773} &     \underline{0.6052} &     \underline{0.5676} \\
wine\_quality   &     0.1292 &     0.2983 &     0.2097 &     \underline{0.2558} &     \underline{0.2774} &     0.2460 &     \underline{0.2537} &     0.2163 &     0.1487 &     0.2244 &     0.2533 &     0.2741 &     \underline{0.2731} &     0.2534 \\
letter\_img     &     0.9722 &     0.9526 &     0.9086 &     0.9410 &     0.9608 &     0.9293 &     \underline{0.9531} &     0.9128 &     0.9661 &     0.9673 &     \underline{0.9556} &     \underline{0.9610} &     \underline{0.9547} &     0.9491 \\
yeast\_me2      &     0.2296 &     0.3192 &     0.2705 &     0.3043 &     0.3621 &     0.2943 &     0.3018 &     0.3227 &     0.2952 &     0.2890 &     \underline{0.3364} &     \underline{0.3759} &     \underline{0.3057} &     \underline{0.3279} \\
ozone\_level    &     0.1608 &     0.2528 &     0.2086 &     0.2087 &     0.2270 &     \underline{0.2516} &     \underline{0.2095} &     0.2108 &     0.2528 &     0.2352 &     \underline{0.2111} &     \underline{0.2443} &     0.2056 &     0.2046 \\
abalone\_19     &     0.0000 &     0.0277 &     0.0500 &     0.0377 &     \underline{0.0482} &     0.0289 &     0.0408 &     0.0366 &     0.0212 &     0.0312 &     \underline{0.0512} &     0.0452 &     \underline{0.0434} &     \underline{0.0498} \\ \hline
\textbf{mean}   &     0.3988 &     0.4790 &     0.4767 &     0.4751 &     0.4888 &     0.4664 &     0.4729 &     0.4817 &     0.4530 &     0.4938 &     \textcolor{blue}{\textbf{\underline{0.4964}}} &     \textcolor{red}{\textbf{\underline{0.5032}}} &     \underline{0.4878} &     \underline{0.4927} \\
\textbf{rank}   &    11.5714 &     7.3095 &     8.0476 &     9.0000 &     \textcolor{blue}{\textbf{4.6905}} &     9.7143 &     9.2381 &     7.5714 &     8.5476 &     6.2381 &     \underline{5.3333} &     \textcolor{red}{\textbf{\underline{3.6429}}} &     \underline{7.4286} &     \underline{6.6667} \\ \bottomrule

\end{tabular}

}

\end{table*}


% ecoli          &      0.5780 &     0.5501 &     0.5864 &     0.5822 &     0.5853 &     0.5781 &     0.5705 &     0.5980 &     0.6336 &     0.5827 &      \underline{0.6275} &        \underline{0.6151} & 0.0000 & 0.0000 \\
% optical\_digits &      0.9670 &     0.9491 &     0.9427 &     0.9415 &     \underline{0.9559} &     0.9439 &     0.9442 &     0.9376 &     0.9491 &     0.9618 &      \underline{0.9443} &        0.9557  & 0.0000 & 0.0000 \\
% pen\_digits     &      0.9927 &     0.9906 &     0.9895 &     0.9906 &     0.9925 &     0.9900 &     0.9917 &     0.9907 &     0.9922 &     0.9928 &      \underline{0.9915} &        \underline{0.9925}  & 0.0000 & 0.0000 \\
% abalone        &      0.1808 &     0.3326 &     0.3842 &     0.3501 &     0.3586 &     0.3727 &     0.3448 &     0.3753 &     0.3281 &     0.3078 &      \underline{0.3698} &        \underline{0.3725}  & 0.0000 & 0.0000 \\
% sick\_euthyroid &      0.5565 &     0.5694 &     0.5872 &     0.5708 &     0.5684 &     0.5246 &     0.5650 &     0.5654 &     0.6081 &     0.5800 &      \underline{0.6049} &        \underline{0.5981}  & 0.0000 & 0.0000 \\
% spectrometer   &      0.7618 &     0.8493 &     0.8382 &     0.8430 &     \underline{0.8543} &     0.8274 &     0.8423 &     0.8551 &     0.7968 &     0.8209 &      \underline{0.8548} &        0.8485  & 0.0000 & 0.0000 \\
% car\_eval\_34    &      0.6018 &     0.5830 &     0.5718 &     0.5774 &     0.5913 &     0.5886 &     0.5851 &     0.6490 &     0.5830 &     0.7165 &      \underline{0.6296} &        \underline{0.6081}  & 0.0000 & 0.0000 \\
% us\_crime       &      0.3676 &     0.4429 &     0.4404 &     0.4188 &     0.4567 &     0.4346 &     0.4144 &     0.4062 &     0.4429 &     0.4634 &      \underline{0.4313} &        \underline{0.4687}  & 0.0000 & 0.0000 \\
% yeast\_ml8      &      0.0375 &     0.1426 &     0.1613 &     0.1592 &     \underline{0.1659} &     0.1542 &     0.1578 &     0.1603 &     0.1426 &     0.1643 &      \underline{0.1598} &        0.1658  & 0.0000 & 0.0000 \\
% scene          &      0.1004 &     0.2500 &     0.2499 &     \underline{0.2386} &     0.2471 &     0.2452 &     0.2309 &     0.2364 &     0.1101 &     0.2579 &      0.2251 &        \underline{0.2482}  & 0.0000 & 0.0000 \\
% libras\_move    &      0.6997 &     0.8031 &     0.7702 &     \underline{0.7672} &     \underline{0.7661} &     0.7362 &     0.7519 &     0.7874 &     0.8031 &     0.8029 &      0.7560 &        0.7568  & 0.0000 & 0.0000 \\
% thyroid\_sick   &      0.4966 &     0.5239 &     0.5246 &     0.5255 &     0.5307 &     0.4620 &     0.5214 &     0.5245 &     0.5095 &     0.5031 &      \underline{0.5504} &        \underline{0.5459}  & 0.0000 & 0.0000 \\
% coil\_2000      &      0.0457 &     0.1745 &     0.1726 &     0.1709 &     \underline{0.1759} &     0.1677 &     0.1711 &     0.1748 &     0.0533 &     0.1168 &      \underline{0.1714} &        0.1748  & 0.0000 & 0.0000 \\
% solar\_flare\_m0 &      0.0510 &     0.2192 &     0.2043 &     0.2077 &     0.2262 &     0.2280 &     0.2188 &     0.2120 &     0.0486 &     0.2126 &      \underline{0.2189} &        \underline{0.2337}  & 0.0000 & 0.0000 \\
% oil            &      0.3156 &     0.4467 &     0.4592 &     0.4428 &     0.4674 &     0.3784 &     0.4240 &     0.4191 &     0.4467 &     0.4626 &      \underline{0.5074} &        \underline{0.5062}  & 0.0000 & 0.0000 \\
% car\_eval\_4     &      0.1294 &     0.3815 &     0.4810 &     0.4443 &     0.4472 &     0.4121 &     0.4371 &     0.5240 &     0.3815 &     0.6771 &      \underline{0.5749} &        \underline{0.5773}  & 0.0000 & 0.0000 \\
% wine\_quality   &      0.1292 &     0.2983 &     0.2097 &     \underline{0.2558} &     \underline{0.2774} &     0.2460 &     0.2537 &     0.2163 &     0.1487 &     0.2244 &      0.2533 &        0.2741  & 0.0000 & 0.0000 \\
% letter\_img     &      0.9722 &     0.9526 &     0.9086 &     0.9410 &     0.9608 &     0.9293 &     0.9531 &     0.9128 &     0.9661 &     0.9673 &      \underline{0.9556} &        \underline{0.9610}  & 0.0000 & 0.0000 \\
% yeast\_me2      &      0.2296 &     0.3192 &     0.2705 &     0.3043 &     0.3621 &     0.2943 &     0.3018 &     0.3227 &     0.2952 &     0.2890 &      \underline{0.3364} &        \underline{0.3759}  & 0.0000 & 0.0000 \\
% ozone\_level    &      0.1608 &     0.2528 &     0.2086 &     0.2087 &     0.2270 &     0.2516 &     0.2095 &     0.2108 &     0.2528 &     0.2352 &      \underline{0.2111} &        \underline{0.2443}  & 0.0000 & 0.0000 \\
% abalone\_19     &      0.0000 &     0.0277 &     0.0500 &     0.0377 &     \underline{0.0482} &     0.0289 &     0.0408 &     0.0366 &     0.0212 &     0.0312 &      \underline{0.0512} &        0.0452  & 0.0000 & 0.0000 \\ \hline \hline
% \textbf{mean}           &      0.3988 &     0.4790 &     0.4767 &     0.4751 &     0.4888 &     0.4664 &     0.4729 &     0.4817 &     0.4530 &     0.4938 &      \textcolor{blue}{\underline{\textbf{0.4964}}} &        \textcolor{red}{\underline{\textbf{0.5032}}}  & 0.0000 & 0.0000 \\
% \textbf{rank}           &      9.9048 &     6.2619 &     6.9524 &     7.5714 &     \textcolor{blue}{\textbf{4.0714}} &     8.2857 &     7.9048 &     6.4286 &     7.3571 &     5.2857 &      \underline{4.7619} &        \textcolor{red}{\underline{\textbf{3.2143}}}  & 0.0000 & 0.0000 \\ \hline

==> tables/datasets_twocol.tex <==
\begin{table*}[h!]
\centering
\caption{Benchmark datasets and their properties.} % two columns?
\label{table:datasets}

%\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lrrrrr|lrrrrr} \toprule
  \textbf{Dataset} &\textbf{Features} &\textbf{Size} &\textbf{Minor} &\textbf{Major} & \textbf{Ratio} & \textbf{Dataset} & \textbf{Features} &\textbf{Size} &\textbf{Minor} &\textbf{Major} &\textbf{Ratio} \\ \midrule
    ecoli & 7 &336 & 35 &301 &9 & thyroid\_sick &52 & 3772 &231 & 3541 & 16 \\
    optical\_digits &64 & 5620 &554 & 5066 & 10 & coil\_2000 &85 & 9822 &586 & 9236 & 16 \\
    pen\_digits &16 &10992 & 1055 & 9937 & 10 & solar\_flare\_m0 &32 & 1389 & 68 & 1321 & 20 \\
    abalone &10 & 4177 &391 & 3786 & 10 & oil &49 &937 & 41 &896 & 22 \\
    sick\_euthyroid &42 & 3163 &293 & 2870 & 10 & car\_eval\_4 &21 & 1728 & 65 & 1663 & 26 \\
    spectrometer &93 &531 & 45 &486 & 11 & wine\_quality &11 & 4898 &183 & 4715 & 26 \\
    car\_eval\_34 &21 & 1728 &134 & 1594 & 12 & letter\_img &16 &20000 &734 &19266 & 27 \\
    us\_crime & 100 & 1994 &150 & 1844 & 13 & yeast\_me2 & 8 & 1484 & 51 & 1433 & 29 \\
    yeast\_ml8 & 103 & 2417 &178 & 2239 & 13 & ozone\_level &72 & 2536 & 73 & 2463 & 34 \\
    scene & 294 & 2407 &177 & 2230 & 13 & abalone\_19 &10 & 4177 & 32 & 4145 &130 \\ 
    libras\_move &90 &360 & 24 &336 & 14 & & & & & & \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/results_dt_f1.tex <==
\begin{table*}[h!]
\label{table:gb_f1}

\caption{Classification results on benchmark datasets for the decision tree classifier. F1 score averaged over $2$ repeats of $5$-fold (outer) cross-validation is reported. \textcolor{red}{\textbf{Best}} and \textcolor{blue}{\textbf{second-best}} results are highlighted.}

\vspace{-0.5em}

\centering

\renewcommand{\arraystretch}{1.27}

\resizebox{\textwidth}{!}{

\begin{tabular}{l|rrrrrrrrrr|rr}
\hline
 & \fontsize{9}{10}\selectfont\textbf{Imbalanced} & \fontsize{9}{10}\selectfont\textbf{Random} & \fontsize{9}{10}\selectfont\textbf{Global} & \fontsize{9}{10}\selectfont\textbf{SMOTE} & \fontsize{9}{10}\selectfont\textbf{B-SMOTE} & \fontsize{9}{10}\selectfont\textbf{Safelevel} & \fontsize{9}{10}\selectfont\textbf{ADASYN} & \fontsize{9}{10}\selectfont\textbf{MWMOTE} & \fontsize{9}{10}\selectfont\textbf{DBSMOTE} & \fontsize{9}{10}\selectfont\textbf{LVQ} & \fontsize{9}{10}\selectfont\textbf{Simplicial} & \fontsize{9}{10}\selectfont\textbf{B-Simplicial} \\ \hline \hline

ecoli &     0.5481 &     0.5274 &     0.5399 &     0.5348 &     0.5373 &     0.5745 &     0.5370 &     0.5587 &     0.5552 &     0.5504 &     0.5338 &     0.5409 \\
optical\_digits &     0.6309 &     0.5627 &     0.5551 &     0.5668 &     0.5365 &     0.5578 &     0.5212 &     0.5579 &     0.5632 &     0.5498 &     0.5581 &     0.5319 \\
pen\_digits &     0.7525 &     0.6159 &     0.5578 &     0.6135 &     0.5468 &     0.6106 &     0.6731 &     0.5893 &     0.6068 &     0.5970 &     0.6266 &     0.5373 \\
abalone &     0.0000 &     0.3658 &     0.3719 &     0.3709 &     0.3703 &     0.3786 &     0.3670 &     0.3728 &     0.3774 &     0.3398 &     0.3785 &     0.3858 \\
sick\_euthyroid &     0.8567 &     0.7613 &     0.8322 &     0.8283 &     0.8242 &     0.7445 &     0.8370 &     0.8369 &     0.8337 &     0.7466 &     0.8268 &     0.8350 \\
spectrometer &     0.6649 &     0.6088 &     0.5149 &     0.6025 &     0.5957 &     0.5954 &     0.5918 &     0.5435 &     0.6099 &     0.6458 &     0.6550 &     0.6080 \\
car\_eval\_34 &     0.4483 &     0.3770 &     0.5174 &     0.4175 &     0.4140 &     0.4363 &     0.3948 &     0.4135 &     0.3652 &     0.3987 &     0.4552 &     0.4731 \\
us\_crime &     0.3990 &     0.4131 &     0.4181 &     0.4293 &     0.4533 &     0.4349 &     0.4279 &     0.4088 &     0.4334 &     0.3425 &     0.4034 &     0.4407 \\
yeast\_ml8 &     0.0054 &     0.1305 &     0.1513 &     0.1460 &     0.1589 &     0.1462 &     0.1381 &     0.1513 &     0.1440 &     0.1140 &     0.1517 &     0.1514 \\
scene &     0.1492 &     0.2230 &     0.2024 &     0.2137 &     0.2085 &     0.2368 &     0.2061 &     0.2163 &     0.0554 &     0.0736 &     0.2002 &     0.2233 \\
libras\_move &     0.3541 &     0.5478 &     0.6010 &     0.5739 &     0.5384 &     0.5055 &     0.5154 &     0.5756 &     0.6092 &     0.5819 &     0.5754 &     0.6357 \\
thyroid\_sick &     0.8175 &     0.6487 &     0.7761 &     0.7014 &     0.7161 &     0.6142 &     0.6869 &     0.7379 &     0.8234 &     0.6612 &     0.7761 &     0.8049 \\
coil\_2000 &     0.0166 &     0.2127 &     0.1963 &     0.1796 &     0.1891 &     0.1922 &     0.1949 &     0.1970 &     0.0852 &     0.0220 &     0.1742 &     0.1875 \\
solar\_flare\_m0 &     0.0845 &     0.1824 &     0.1989 &     0.1689 &     0.1684 &     0.1679 &     0.1647 &     0.1222 &     0.0836 &     0.1965 &     0.1561 &     0.1479 \\
oil &     0.4178 &     0.2609 &     0.3429 &     0.2850 &     0.3577 &     0.3184 &     0.2774 &     0.2500 &     0.3056 &     0.3310 &     0.3570 &     0.4499 \\
car\_eval\_4 &     0.0000 &     0.4090 &     0.4132 &     0.4090 &     0.4090 &     0.4090 &     0.4090 &     0.4090 &     0.4090 &     0.3852 &     0.3922 &     0.4090 \\
wine\_quality &     0.1498 &     0.2338 &     0.1424 &     0.1815 &     0.1641 &     0.1949 &     0.1377 &     0.1569 &     0.1388 &     0.2437 &     0.1664 &     0.1810 \\
letter\_img &     0.6802 &     0.3643 &     0.5952 &     0.4351 &     0.3734 &     0.4373 &     0.3653 &     0.4305 &     0.6415 &     0.4674 &     0.6541 &     0.4270 \\
yeast\_me2 &     0.2514 &     0.2196 &     0.2218 &     0.2167 &     0.2648 &     0.2061 &     0.2095 &     0.2335 &     0.1096 &     0.2659 &     0.2349 &     0.2687 \\
ozone\_level &     0.0190 &     0.1429 &     0.1481 &     0.1523 &     0.1871 &     0.1666 &     0.1582 &     0.1836 &     0.1579 &     0.1558 &     0.2076 &     0.1887 \\
abalone\_19 &     0.0000 &     0.0346 &     0.0227 &     0.0350 &     0.0608 &     0.0447 &     0.0357 &     0.0564 &     0.0425 &     0.0319 &     0.0328 &     0.0539 \\ \hline \hline
mean &     0.3450 &     0.3734 &     0.3962 &     0.3839 &     0.3845 &     0.3796 &     0.3737 &     0.3810 &     0.3786 &     0.3667 &     \textcolor{red}{\textbf{0.4055}} &     \textcolor{blue}{\textbf{0.4039}} \\
rank &     7.0000 &     7.5000 &     6.0952 &     6.5952 &     6.1190 &     6.0714 &     7.9286 &     6.2143 &     6.5952 &     7.5714 &     \textcolor{blue}{\textbf{5.7619}} &     \textcolor{red}{\textbf{4.5476}} \\ \hline

\end{tabular}

}

\end{table*}

==> tables/results_dt_f1_25.tex <==
\begin{table*}[h!]
\caption{Classification results on benchmark datasets for the decision tree classifier. F1 score averaged over $2$ repeats of $5$-fold (outer) cross-validation is reported. \textcolor{red}{\textbf{Best}} and \textcolor{blue}{\textbf{second-best}} results are highlighted.}
\label{table:dt_f1}

\vspace{-0.5em}

\centering

\renewcommand{\arraystretch}{1.27}

\resizebox{\textwidth}{!}{

\begin{tabular}{l|rrrrrrrrrr|rrrr}
\hline
 & \fontsize{8}{9}\selectfont\textbf{Imbalanced} & \fontsize{8}{9}\selectfont\textbf{Random} & \fontsize{8}{9}\selectfont\textbf{Global} & \fontsize{8}{9}\selectfont\textbf{SMOTE} & \fontsize{8}{9}\selectfont\textbf{Border.} & \fontsize{8}{9}\selectfont\textbf{Safelevel} & \fontsize{8}{9}\selectfont\textbf{ADASYN} & \fontsize{8}{9}\selectfont\textbf{MWMOTE} & \fontsize{8}{9}\selectfont\textbf{DBSMOTE} & \fontsize{8}{9}\selectfont\textbf{LVQ} & \fontsize{8}{9}\selectfont\textbf{Simplicial} & \fontsize{8}{9}\selectfont\textbf{S-Border.} & \fontsize{8}{9}\selectfont\textbf{S-Safe.} & \fontsize{8}{9}\selectfont\textbf{S-ADASYN} \\  \hline \hline

ecoli &     0.5481 &     0.5274 &     0.5399 &     0.5348 &     0.5373 &     0.5745 &     0.5370 &     0.5587 &     0.5552 &     0.5504 &     0.5338 &     0.5409 &     0.4964 &     0.5317 \\
optical\_digits &     0.6309 &     0.5627 &     0.5551 &     0.5668 &     0.5365 &     0.5578 &     0.5212 &     0.5579 &     0.5632 &     0.5498 &     0.5581 &     0.5319 &     0.5616 &     0.5723 \\
pen\_digits &     0.7525 &     0.6159 &     0.5578 &     0.6135 &     0.5468 &     0.6106 &     0.6731 &     0.5893 &     0.6068 &     0.5970 &     0.6266 &     0.5373 &     0.6284 &     0.6368 \\
abalone &     0.0000 &     0.3658 &     0.3719 &     0.3709 &     0.3703 &     0.3786 &     0.3670 &     0.3728 &     0.3774 &     0.3398 &     0.3785 &     0.3858 &     0.3747 &     0.3690 \\
sick\_euthyroid &     0.8567 &     0.7613 &     0.8322 &     0.8283 &     0.8242 &     0.7445 &     0.8370 &     0.8369 &     0.8337 &     0.7466 &     0.8268 &     0.8350 &     0.7987 &     0.8362 \\
spectrometer &     0.6649 &     0.6088 &     0.5149 &     0.6025 &     0.5957 &     0.5954 &     0.5918 &     0.5435 &     0.6099 &     0.6458 &     0.6550 &     0.6080 &     0.6712 &     0.6225 \\
car\_eval\_34 &     0.4483 &     0.3770 &     0.5174 &     0.4175 &     0.4140 &     0.4363 &     0.3948 &     0.4135 &     0.3652 &     0.3987 &     0.4552 &     0.4731 &     0.4552 &     0.4430 \\
us\_crime &     0.3990 &     0.4131 &     0.4181 &     0.4293 &     0.4533 &     0.4349 &     0.4279 &     0.4088 &     0.4334 &     0.3425 &     0.4034 &     0.4407 &     0.4264 &     0.4222 \\
yeast\_ml8 &     0.0054 &     0.1305 &     0.1513 &     0.1460 &     0.1589 &     0.1462 &     0.1381 &     0.1513 &     0.1440 &     0.1140 &     0.1517 &     0.1514 &     0.1550 &     0.1467 \\
scene &     0.1492 &     0.2230 &     0.2024 &     0.2137 &     0.2085 &     0.2368 &     0.2061 &     0.2163 &     0.0554 &     0.0736 &     0.2002 &     0.2233 &     0.1903 &     0.1877 \\
libras\_move &     0.3541 &     0.5478 &     0.6010 &     0.5739 &     0.5384 &     0.5055 &     0.5154 &     0.5756 &     0.6092 &     0.5819 &     0.5754 &     0.6357 &     0.5247 &     0.5050 \\
thyroid\_sick &     0.8175 &     0.6487 &     0.7761 &     0.7014 &     0.7161 &     0.6142 &     0.6869 &     0.7379 &     0.8234 &     0.6612 &     0.7761 &     0.8049 &     0.7877 &     0.7760 \\
coil\_2000 &     0.0166 &     0.2127 &     0.1963 &     0.1796 &     0.1891 &     0.1922 &     0.1949 &     0.1970 &     0.0852 &     0.0220 &     0.1742 &     0.1875 &     0.1728 &     0.1743 \\
solar\_flare\_m0 &     0.0845 &     0.1824 &     0.1989 &     0.1689 &     0.1684 &     0.1679 &     0.1647 &     0.1222 &     0.0836 &     0.1965 &     0.1561 &     0.1479 &     0.1321 &     0.0906 \\
oil &     0.4178 &     0.2609 &     0.3429 &     0.2850 &     0.3577 &     0.3184 &     0.2774 &     0.2500 &     0.3056 &     0.3310 &     0.3570 &     0.4499 &     0.2720 &     0.3987 \\
car\_eval\_4 &     0.0000 &     0.4090 &     0.4132 &     0.4090 &     0.4090 &     0.4090 &     0.4090 &     0.4090 &     0.4090 &     0.3852 &     0.3922 &     0.4090 &     0.3922 &     0.3922 \\
wine\_quality &     0.1498 &     0.2338 &     0.1424 &     0.1815 &     0.1641 &     0.1949 &     0.1377 &     0.1569 &     0.1388 &     0.2437 &     0.1664 &     0.1810 &     0.1670 &     0.1395 \\
letter\_img &     0.6802 &     0.3643 &     0.5952 &     0.4351 &     0.3734 &     0.4373 &     0.3653 &     0.4305 &     0.6415 &     0.4674 &     0.6541 &     0.4270 &     0.5950 &     0.4592 \\
yeast\_me2 &     0.2514 &     0.2196 &     0.2218 &     0.2167 &     0.2648 &     0.2061 &     0.2095 &     0.2335 &     0.1096 &     0.2659 &     0.2349 &     0.2687 &     0.2330 &     0.2256 \\
ozone\_level &     0.0190 &     0.1429 &     0.1481 &     0.1523 &     0.1871 &     0.1666 &     0.1582 &     0.1836 &     0.1579 &     0.1558 &     0.2076 &     0.1887 &     0.1888 &     0.2058 \\
abalone\_19 &     0.0000 &     0.0346 &     0.0227 &     0.0350 &     0.0608 &     0.0447 &     0.0357 &     0.0564 &     0.0425 &     0.0319 &     0.0328 &     0.0539 &     0.0413 &     0.0336 \\ \hline \hline
mean &     0.3450 &     0.3734 &     0.3962 &     0.3839 &     0.3845 &     0.3796 &     0.3737 &     0.3810 &     0.3786 &     0.3667 &     \textcolor{red}{\textbf{0.4055}} &     \textcolor{blue}{\textbf{0.4039}} &     0.3935 &     0.3890 \\
rank &     8.0952 &     8.7857 &     7.0476 &     7.5952 &     6.9762 &     7.1190 &     9.0238 &     7.2619 &     7.6905 &     8.9524 &     \textcolor{blue}{\textbf{6.5476}} &     \textcolor{red}{\textbf{5.1190}} &     7.0714 &     7.7143 \\ \hline

\end{tabular}

}

\end{table*}

==> tables/results_lr_f1.tex <==
\begin{table*}[h!]
\label{table:gb_f1}

\caption{Classification results on benchmark datasets for the logistic regression classifier. F1 score averaged over $2$ repeats of $5$-fold (outer) cross-validation is reported. \textcolor{red}{\textbf{Best}} and \textcolor{blue}{\textbf{second-best}} results are highlighted.}

\vspace{-0.5em}

\centering

\renewcommand{\arraystretch}{1.27}

\resizebox{\textwidth}{!}{

\begin{tabular}{l|rrrrrrrrrr|rr}
\hline
 & \fontsize{9}{10}\selectfont\textbf{Imbalanced} & \fontsize{9}{10}\selectfont\textbf{Random} & \fontsize{9}{10}\selectfont\textbf{Global} & \fontsize{9}{10}\selectfont\textbf{SMOTE} & \fontsize{9}{10}\selectfont\textbf{B-SMOTE} & \fontsize{9}{10}\selectfont\textbf{Safelevel} & \fontsize{9}{10}\selectfont\textbf{ADASYN} & \fontsize{9}{10}\selectfont\textbf{MWMOTE} & \fontsize{9}{10}\selectfont\textbf{DBSMOTE} & \fontsize{9}{10}\selectfont\textbf{LVQ} & \fontsize{9}{10}\selectfont\textbf{Simplicial} & \fontsize{9}{10}\selectfont\textbf{B-Simplicial} \\ \hline \hline

ecoli &     0.5418 &     0.6116 &     0.6249 &     0.6016 &     0.6266 &     0.6067 &     0.5897 &     0.6503 &     0.6809 &     0.5792 &     0.6530 &     0.6407 \\
optical\_digits &     0.8434 &     0.7642 &     0.7921 &     0.7958 &     0.7559 &     0.7863 &     0.7518 &     0.7862 &     0.7702 &     0.8383 &     0.8147 &     0.7614 \\
pen\_digits &     0.7917 &     0.7219 &     0.7398 &     0.7343 &     0.5640 &     0.7302 &     0.5671 &     0.7036 &     0.7404 &     0.7526 &     0.7436 &     0.5620 \\
abalone &     0.0150 &     0.3587 &     0.3629 &     0.3627 &     0.3758 &     0.3666 &     0.3577 &     0.3769 &     0.3676 &     0.3357 &     0.3748 &     0.3751 \\
sick\_euthyroid &     0.6720 &     0.6103 &     0.6243 &     0.6317 &     0.6273 &     0.5821 &     0.6090 &     0.6310 &     0.7122 &     0.6933 &     0.7271 &     0.6952 \\
spectrometer &     0.8374 &     0.8440 &     0.8734 &     0.8502 &     0.8465 &     0.8319 &     0.8422 &     0.8502 &     0.8409 &     0.7429 &     0.8636 &     0.8452 \\
car\_eval\_34 &     0.9125 &     0.8806 &     0.8844 &     0.8835 &     0.8842 &     0.7881 &     0.8828 &     0.8827 &     0.8734 &     0.8820 &     0.8917 &     0.8904 \\
us\_crime &     0.5354 &     0.4674 &     0.4891 &     0.4922 &     0.5198 &     0.4875 &     0.4767 &     0.4877 &     0.4717 &     0.4781 &     0.4950 &     0.5195 \\
yeast\_ml8 &     0.0319 &     0.1395 &     0.1420 &     0.1398 &     0.1417 &     0.1442 &     0.1434 &     0.1483 &     0.1424 &     0.1280 &     0.1365 &     0.1421 \\
scene &     0.1934 &     0.2481 &     0.2456 &     0.2480 &     0.2427 &     0.2348 &     0.2426 &     0.2552 &     0.2241 &     0.2338 &     0.2334 &     0.2576 \\
libras\_move &     0.8179 &     0.7357 &     0.7520 &     0.7710 &     0.7876 &     0.7128 &     0.7621 &     0.7448 &     0.7448 &     0.6710 &     0.8356 &     0.8254 \\
thyroid\_sick &     0.6554 &     0.4822 &     0.5054 &     0.5059 &     0.5215 &     0.4234 &     0.4940 &     0.5109 &     0.6449 &     0.6393 &     0.6413 &     0.6641 \\
coil\_2000 &     0.0197 &     0.1988 &     0.2010 &     0.1931 &     0.1977 &     0.1929 &     0.1914 &     0.1999 &     0.1229 &     0.1860 &     0.2058 &     0.2091 \\
solar\_flare\_m0 &     0.1122 &     0.2046 &     0.1979 &     0.1917 &     0.1986 &     0.2008 &     0.1904 &     0.1962 &     0.1253 &     0.1922 &     0.1923 &     0.1986 \\
oil &     0.5085 &     0.4536 &     0.4976 &     0.4639 &     0.4523 &     0.3881 &     0.4698 &     0.4559 &     0.4381 &     0.4371 &     0.4998 &     0.4900 \\
car\_eval\_4 &     0.8469 &     0.8303 &     0.8485 &     0.8436 &     0.8462 &     0.7957 &     0.8485 &     0.8533 &     0.8269 &     0.8471 &     0.8589 &     0.8559 \\
wine\_quality &     0.0892 &     0.1760 &     0.1818 &     0.1765 &     0.1814 &     0.1825 &     0.1772 &     0.1870 &     0.1801 &     0.1705 &     0.1788 &     0.1828 \\
letter\_img &     0.7418 &     0.5540 &     0.5930 &     0.5786 &     0.5051 &     0.5646 &     0.5099 &     0.5656 &     0.6581 &     0.5958 &     0.6480 &     0.5175 \\
yeast\_me2 &     0.2066 &     0.2624 &     0.2631 &     0.2656 &     0.3049 &     0.2622 &     0.2538 &     0.2793 &     0.3381 &     0.2528 &     0.2799 &     0.3422 \\
ozone\_level &     0.1970 &     0.2522 &     0.2703 &     0.2661 &     0.3028 &     0.2363 &     0.2624 &     0.2843 &     0.2495 &     0.2862 &     0.3077 &     0.3253 \\
abalone\_19 &     0.0000 &     0.0463 &     0.0471 &     0.0474 &     0.0556 &     0.0473 &     0.0473 &     0.0534 &     0.0408 &     0.0477 &     0.0580 &     0.0589 \\ \hline \hline
mean &     0.4557 &     0.4687 &     0.4827 &     0.4782 &     0.4733 &     0.4555 &     0.4605 &     0.4811 &     0.4854 &     0.4757 &     \textcolor{red}{\textbf{0.5066}} &     \textcolor{blue}{\textbf{0.4933}} \\
rank &     7.2857 &     8.3333 &     5.5476 &     6.5476 &     5.9524 &     8.3333 &     8.4524 &     5.0476 &     7.2143 &     7.9524 &     \textcolor{red}{\textbf{3.6190}} &     \textcolor{blue}{\textbf{3.7143}} \\ \hline

\end{tabular}

}

\end{table*}

==> tables/results_lr_f1_25.tex <==
\begin{table*}[h!]

\caption{Classification results on benchmark datasets for the logistic regression classifier. F1 score averaged over $2$ repeats of $5$-fold (outer) cross-validation is reported. \textcolor{red}{\textbf{Best}} and \textcolor{blue}{\textbf{second-best}} results are highlighted.}
\label{table:lr_f1}

\vspace{-0.5em}

\centering

\renewcommand{\arraystretch}{1.27}

\resizebox{\textwidth}{!}{

\begin{tabular}{l|rrrrrrrrrr|rrrr}
\hline
 & \fontsize{8}{9}\selectfont\textbf{Imbalanced} & \fontsize{8}{9}\selectfont\textbf{Random} & \fontsize{8}{9}\selectfont\textbf{Global} & \fontsize{8}{9}\selectfont\textbf{SMOTE} & \fontsize{8}{9}\selectfont\textbf{Border.} & \fontsize{8}{9}\selectfont\textbf{Safelevel} & \fontsize{8}{9}\selectfont\textbf{ADASYN} & \fontsize{8}{9}\selectfont\textbf{MWMOTE} & \fontsize{8}{9}\selectfont\textbf{DBSMOTE} & \fontsize{8}{9}\selectfont\textbf{LVQ} & \fontsize{8}{9}\selectfont\textbf{Simplicial} & \fontsize{8}{9}\selectfont\textbf{S-Border.} & \fontsize{8}{9}\selectfont\textbf{S-Safe.} & \fontsize{8}{9}\selectfont\textbf{S-ADASYN} \\  \hline \hline

ecoli &     0.5418 &     0.6116 &     0.6249 &     0.6016 &     0.6266 &     0.6067 &     0.5897 &     0.6503 &     0.6809 &     0.5792 &     0.6530 &     0.6407 &     0.5998 &     0.6575 \\
optical\_digits &     0.8434 &     0.7642 &     0.7921 &     0.7958 &     0.7559 &     0.7863 &     0.7518 &     0.7862 &     0.7702 &     0.8383 &     0.8147 &     0.7614 &     0.7960 &     0.7813 \\
pen\_digits &     0.7917 &     0.7219 &     0.7398 &     0.7343 &     0.5640 &     0.7302 &     0.5671 &     0.7036 &     0.7404 &     0.7526 &     0.7436 &     0.5620 &     0.7369 &     0.6305 \\
abalone &     0.0150 &     0.3587 &     0.3629 &     0.3627 &     0.3758 &     0.3666 &     0.3577 &     0.3769 &     0.3676 &     0.3357 &     0.3748 &     0.3751 &     0.3737 &     0.3712 \\
sick\_euthyroid &     0.6720 &     0.6103 &     0.6243 &     0.6317 &     0.6273 &     0.5821 &     0.6090 &     0.6310 &     0.7122 &     0.6933 &     0.7271 &     0.6952 &     0.6494 &     0.6990 \\
spectrometer &     0.8374 &     0.8440 &     0.8734 &     0.8502 &     0.8465 &     0.8319 &     0.8422 &     0.8502 &     0.8409 &     0.7429 &     0.8636 &     0.8452 &     0.8651 &     0.8341 \\
car\_eval\_34 &     0.9125 &     0.8806 &     0.8844 &     0.8835 &     0.8842 &     0.7881 &     0.8828 &     0.8827 &     0.8734 &     0.8820 &     0.8917 &     0.8904 &     0.8891 &     0.8962 \\
us\_crime &     0.5354 &     0.4674 &     0.4891 &     0.4922 &     0.5198 &     0.4875 &     0.4767 &     0.4877 &     0.4717 &     0.4781 &     0.4950 &     0.5195 &     0.5016 &     0.4989 \\
yeast\_ml8 &     0.0319 &     0.1395 &     0.1420 &     0.1398 &     0.1417 &     0.1442 &     0.1434 &     0.1483 &     0.1424 &     0.1280 &     0.1365 &     0.1421 &     0.1323 &     0.1386 \\
scene &     0.1934 &     0.2481 &     0.2456 &     0.2480 &     0.2427 &     0.2348 &     0.2426 &     0.2552 &     0.2241 &     0.2338 &     0.2334 &     0.2576 &     0.2298 &     0.2262 \\
libras\_move &     0.8179 &     0.7357 &     0.7520 &     0.7710 &     0.7876 &     0.7128 &     0.7621 &     0.7448 &     0.7448 &     0.6710 &     0.8356 &     0.8254 &     0.7851 &     0.8135 \\
thyroid\_sick &     0.6554 &     0.4822 &     0.5054 &     0.5059 &     0.5215 &     0.4234 &     0.4940 &     0.5109 &     0.6449 &     0.6393 &     0.6413 &     0.6641 &     0.6152 &     0.6537 \\
coil\_2000 &     0.0197 &     0.1988 &     0.2010 &     0.1931 &     0.1977 &     0.1929 &     0.1914 &     0.1999 &     0.1229 &     0.1860 &     0.2058 &     0.2091 &     0.2023 &     0.2033 \\
solar\_flare\_m0 &     0.1122 &     0.2046 &     0.1979 &     0.1917 &     0.1986 &     0.2008 &     0.1904 &     0.1962 &     0.1253 &     0.1922 &     0.1923 &     0.1986 &     0.1966 &     0.1988 \\
oil &     0.5085 &     0.4536 &     0.4976 &     0.4639 &     0.4523 &     0.3881 &     0.4698 &     0.4559 &     0.4381 &     0.4371 &     0.4998 &     0.4900 &     0.4149 &     0.4856 \\
car\_eval\_4 &     0.8469 &     0.8303 &     0.8485 &     0.8436 &     0.8462 &     0.7957 &     0.8485 &     0.8533 &     0.8269 &     0.8471 &     0.8589 &     0.8559 &     0.8549 &     0.8608 \\
wine\_quality &     0.0892 &     0.1760 &     0.1818 &     0.1765 &     0.1814 &     0.1825 &     0.1772 &     0.1870 &     0.1801 &     0.1705 &     0.1788 &     0.1828 &     0.1793 &     0.1713 \\
letter\_img &     0.7418 &     0.5540 &     0.5930 &     0.5786 &     0.5051 &     0.5646 &     0.5099 &     0.5656 &     0.6581 &     0.5958 &     0.6480 &     0.5175 &     0.6252 &     0.5574 \\
yeast\_me2 &     0.2066 &     0.2624 &     0.2631 &     0.2656 &     0.3049 &     0.2622 &     0.2538 &     0.2793 &     0.3381 &     0.2528 &     0.2799 &     0.3422 &     0.2699 &     0.2994 \\
ozone\_level &     0.1970 &     0.2522 &     0.2703 &     0.2661 &     0.3028 &     0.2363 &     0.2624 &     0.2843 &     0.2495 &     0.2862 &     0.3077 &     0.3253 &     0.2791 &     0.3055 \\
abalone\_19 &     0.0000 &     0.0463 &     0.0471 &     0.0474 &     0.0556 &     0.0473 &     0.0473 &     0.0534 &     0.0408 &     0.0477 &     0.0580 &     0.0589 &     0.0602 &     0.0580 \\ \hline \hline
mean &     0.4557 &     0.4687 &     0.4827 &     0.4782 &     0.4733 &     0.4555 &     0.4605 &     0.4811 &     0.4854 &     0.4757 &     \textcolor{red}{\textbf{0.5066}} &     \textcolor{blue}{\textbf{0.4933}} &     0.4884 &     0.4924 \\
rank &     8.4286 &     9.8095 &     6.7857 &     8.0238 &     7.0952 &     9.7619 &    10.1190 &     6.2857 &     8.4048 &     9.4286 &     \textcolor{red}{\textbf{4.2381}} &     \textcolor{blue}{\textbf{4.3333}} &     6.3810 &     5.9048 \\ \hline

\end{tabular}

}

\end{table*}

==> tables/results_svm_f1.tex <==
\begin{table*}[h!]

\caption{Classification results on benchmark datasets for the SVM classifier with RBF kernel. F1 score averaged over $5$ repeats of $5$-fold (outer) cross-validation is reported. \textcolor{red}{\textbf{Best}} and \textcolor{blue}{\textbf{second-best}} results are highlighted.}
\label{table:svm_rbf_f1}

%\vspace{-0.5em}

\centering

\renewcommand{\arraystretch}{1.15}

\resizebox{\textwidth}{!}{

\begin{tabular}{l|rrrrrrrrrr|rrrr}
\toprule
 & \fontsize{8}{9}\selectfont\textbf{Imbalanced} & \fontsize{8}{9}\selectfont\textbf{Random} & \fontsize{8}{9}\selectfont\textbf{Global} & \fontsize{8}{9}\selectfont\textbf{SMOTE} & \fontsize{8}{9}\selectfont\textbf{Border.} & \fontsize{8}{9}\selectfont\textbf{Safelevel} & \fontsize{8}{9}\selectfont\textbf{ADASYN} & \fontsize{8}{9}\selectfont\textbf{MWMOTE} & \fontsize{8}{9}\selectfont\textbf{DBSMOTE} & \fontsize{8}{9}\selectfont\textbf{LVQ} & \fontsize{8}{9}\selectfont\textbf{Simplicial} & \fontsize{8}{9}\selectfont\textbf{S-Border.} & \fontsize{8}{9}\selectfont\textbf{S-Safe.} & \fontsize{8}{9}\selectfont\textbf{S-ADASYN} \\  \midrule

ecoli &     0.6238 &     0.6033 &     0.6294 &     0.6284 &     0.6130 &     0.6025 &     0.5989 &     0.6148 &     0.6661 &     0.5995 &     0.6794 &     0.6513 &     0.6390 &     0.6817 \\
optical\_digits &     0.9597 &     0.9741 &     0.9766 &     0.9761 &     0.9691 &     0.9755 &     0.9731 &     0.9749 &     0.9753 &     0.9285 &     0.9752 &     0.9711 &     0.9743 &     0.9740 \\
pen\_digits &     0.9918 &     0.9936 &     0.9916 &     0.9935 &     0.9908 &     0.9938 &     0.9902 &     0.9932 &     0.9925 &     0.9915 &     0.9934 &     0.9905 &     0.9938 &     0.9916 \\
abalone &     0.0000 &     0.3810 &     0.4212 &     0.3883 &     0.3880 &     0.3880 &     0.3783 &     0.3892 &     0.3890 &     0.3583 &     0.4029 &     0.4037 &     0.3948 &     0.3913 \\
sick\_euthyroid &     0.1727 &     0.6027 &     0.6524 &     0.6230 &     0.6069 &     0.5785 &     0.6067 &     0.6175 &     0.6347 &     0.6625 &     0.6614 &     0.6469 &     0.6425 &     0.6486 \\
spectrometer &     0.8474 &     0.8130 &     0.8263 &     0.8205 &     0.8171 &     0.8196 &     0.8211 &     0.8175 &     0.8595 &     0.8582 &     0.8467 &     0.8227 &     0.8419 &     0.8571 \\
car\_eval\_34 &     0.8853 &     0.9372 &     0.9436 &     0.9425 &     0.9411 &     0.8958 &     0.9437 &     0.9457 &     0.9372 &     0.9143 &     0.9414 &     0.9465 &     0.9468 &     0.9450 \\
us\_crime &     0.3589 &     0.5066 &     0.4923 &     0.4818 &     0.5016 &     0.5265 &     0.4657 &     0.4730 &     0.5099 &     0.5412 &     0.4727 &     0.4974 &     0.4611 &     0.4669 \\
yeast\_ml8 &     0.0000 &     0.0319 &     0.0044 &     0.0085 &     0.0065 &     0.0761 &     0.0022 &     0.0000 &     0.0319 &     0.0168 &     0.0000 &     0.0022 &     0.0000 &     0.0000 \\
scene &     0.0175 &     0.2866 &     0.2724 &     0.2674 &     0.2711 &     0.2649 &     0.2655 &     0.2556 &     0.0261 &     0.2090 &     0.2599 &     0.2654 &     0.2199 &     0.2587 \\
libras\_move &     0.8148 &     0.8174 &     0.8030 &     0.8063 &     0.8465 &     0.7280 &     0.8133 &     0.8227 &     0.8174 &     0.7913 &     0.8289 &     0.8271 &     0.8189 &     0.8465 \\
thyroid\_sick &     0.0648 &     0.5457 &     0.5880 &     0.5769 &     0.5717 &     0.4731 &     0.5606 &     0.5754 &     0.5517 &     0.5488 &     0.6443 &     0.6395 &     0.6384 &     0.6459 \\
coil\_2000 &     0.0000 &     0.1934 &     0.1869 &     0.1844 &     0.1845 &     0.1808 &     0.1815 &     0.1814 &     0.0154 &     0.1323 &     0.1773 &     0.1765 &     0.1723 &     0.1761 \\
solar\_flare\_m0 &     0.0000 &     0.1673 &     0.1643 &     0.1614 &     0.1482 &     0.1642 &     0.1625 &     0.1407 &     0.0290 &     0.2409 &     0.1465 &     0.1370 &     0.1384 &     0.1438 \\
oil &     0.3702 &     0.4438 &     0.4752 &     0.4475 &     0.4825 &     0.4193 &     0.4421 &     0.4601 &     0.4447 &     0.4975 &     0.4712 &     0.5242 &     0.4354 &     0.4258 \\
car\_eval\_4 &     0.9677 &     0.9557 &     0.9597 &     0.9583 &     0.9583 &     0.8976 &     0.9583 &     0.9597 &     0.9557 &     0.8887 &     0.9652 &     0.9637 &     0.9624 &     0.9667 \\
wine\_quality &     0.0352 &     0.2425 &     0.1959 &     0.2411 &     0.2538 &     0.2369 &     0.2321 &     0.2128 &     0.1430 &     0.2616 &     0.2408 &     0.2533 &     0.2406 &     0.2365 \\
letter\_img &     0.9522 &     0.9452 &     0.9369 &     0.9559 &     0.9548 &     0.9480 &     0.9569 &     0.9602 &     0.9382 &     0.9521 &     0.9637 &     0.9555 &     0.9626 &     0.9659 \\
yeast\_me2 &     0.0139 &     0.2816 &     0.2872 &     0.2947 &     0.3559 &     0.2672 &     0.2881 &     0.3085 &     0.3485 &     0.3095 &     0.3585 &     0.4163 &     0.3137 &     0.3493 \\
ozone\_level &     0.0000 &     0.3095 &     0.2908 &     0.2956 &     0.3150 &     0.2465 &     0.2955 &     0.3024 &     0.3103 &     0.3489 &     0.3250 &     0.3306 &     0.3169 &     0.3250 \\
abalone\_19 &     0.0000 &     0.0444 &     0.0553 &     0.0503 &     0.0474 &     0.0381 &     0.0500 &     0.0497 &     0.0293 &     0.0484 &     0.0555 &     0.0492 &     0.0613 &     0.0541 \\ \hline 
mean &     0.3846 &     0.5274 &     0.5311 &     0.5287 &     0.5345 &     0.5105 &     0.5232 &     0.5264 &     0.5050 &     0.5286 &     \textcolor{blue}{\textbf{0.5433}} &     \textcolor{red}{\textbf{0.5462}} &     0.5321 &     0.5405 \\
rank &    11.7143 &     7.9524 &     6.3571 &     6.7143 &     7.1429 &     9.1905 &     9.0952 &     7.6905 &     8.1905 &     7.8095 &     \textcolor{red}{\textbf{4.9524}} &     \textcolor{blue}{\textbf{5.6667}} &     6.5238 &     6.0000 \\ \bottomrule

\end{tabular}

}

\end{table*}

==> tables/results_svm_linear_f1_25.tex <==
\begin{table*}[h!]
\caption{Classification results on benchmark datasets for the SVM classifier with linear kernel. F1 score averaged over $5$ repeats of $5$-fold (outer) cross-validation is reported. \textcolor{red}{\textbf{Best}} and \textcolor{blue}{\textbf{second-best}} results are highlighted.}
\label{table:svm_linear_f1}

\vspace{-0.5em}

\centering

\renewcommand{\arraystretch}{1.27}

\resizebox{\textwidth}{!}{

\begin{tabular}{l|rrrrrrrrrr|rrrr}
\hline
 & \fontsize{8}{9}\selectfont\textbf{Imbalanced} & \fontsize{8}{9}\selectfont\textbf{Random} & \fontsize{8}{9}\selectfont\textbf{Global} & \fontsize{8}{9}\selectfont\textbf{SMOTE} & \fontsize{8}{9}\selectfont\textbf{Border.} & \fontsize{8}{9}\selectfont\textbf{Safelevel} & \fontsize{8}{9}\selectfont\textbf{ADASYN} & \fontsize{8}{9}\selectfont\textbf{MWMOTE} & \fontsize{8}{9}\selectfont\textbf{DBSMOTE} & \fontsize{8}{9}\selectfont\textbf{LVQ} & \fontsize{8}{9}\selectfont\textbf{Simplicial} & \fontsize{8}{9}\selectfont\textbf{S-Border.} & \fontsize{8}{9}\selectfont\textbf{S-Safe.} & \fontsize{8}{9}\selectfont\textbf{S-ADASYN} \\  \hline \hline

ecoli &     0.5410 &     0.6193 &     0.6218 &     0.6295 &     0.6069 &     0.6076 &     0.6077 &     0.6364 &     0.6807 &     0.5803 &     0.6627 &     0.6311 &     0.5841 &     0.6452 \\
optical\_digits &     0.8463 &     0.7664 &     0.7912 &     0.7910 &     0.7453 &     0.7881 &     0.7427 &     0.7881 &     0.7677 &     0.8350 &     0.8105 &     0.7501 &     0.7995 &     0.7799 \\
pen\_digits &     0.7948 &     0.7251 &     0.7404 &     0.7344 &     0.5471 &     0.7330 &     0.5601 &     0.7029 &     0.7373 &     0.7484 &     0.7426 &     0.5480 &     0.7399 &     0.6201 \\
abalone &     0.0020 &     0.3492 &     0.3547 &     0.3562 &     0.3665 &     0.3595 &     0.3493 &     0.3692 &     0.3610 &     0.3322 &     0.3685 &     0.3696 &     0.3665 &     0.3639 \\
sick\_euthyroid &     0.6923 &     0.5985 &     0.6183 &     0.6275 &     0.6229 &     0.5712 &     0.6016 &     0.6269 &     0.7030 &     0.6873 &     0.7084 &     0.6911 &     0.6478 &     0.6943 \\
spectrometer &     0.8199 &     0.7896 &     0.8118 &     0.7984 &     0.8106 &     0.8019 &     0.7969 &     0.7937 &     0.8165 &     0.6863 &     0.8239 &     0.8187 &     0.8177 &     0.8183 \\
car\_eval\_34 &     0.9228 &     0.9083 &     0.9067 &     0.9050 &     0.9030 &     0.7982 &     0.9050 &     0.9048 &     0.9078 &     0.8781 &     0.9143 &     0.9088 &     0.9151 &     0.9120 \\
us\_crime &     0.5121 &     0.4440 &     0.4631 &     0.4532 &     0.4871 &     0.4873 &     0.4412 &     0.4537 &     0.4487 &     0.4707 &     0.4887 &     0.4857 &     0.4669 &     0.4762 \\
yeast\_ml8 &     0.0022 &     0.1433 &     0.1441 &     0.1403 &     0.1435 &     0.1432 &     0.1354 &     0.1445 &     0.1471 &     0.1281 &     0.1397 &     0.1434 &     0.1392 &     0.1387 \\
scene &     0.1962 &     0.2222 &     0.2282 &     0.2249 &     0.2308 &     0.2363 &     0.2241 &     0.2262 &     0.1970 &     0.2145 &     0.2243 &     0.2369 &     0.2184 &     0.2173 \\
libras\_move &     0.7765 &     0.7342 &     0.7396 &     0.7455 &     0.7507 &     0.7352 &     0.7415 &     0.7318 &     0.7259 &     0.7182 &     0.7776 &     0.7609 &     0.7497 &     0.7721 \\
thyroid\_sick &     0.6130 &     0.4598 &     0.4800 &     0.4941 &     0.5178 &     0.4161 &     0.4768 &     0.4960 &     0.6318 &     0.6330 &     0.6553 &     0.6738 &     0.6054 &     0.6604 \\
coil\_2000 &     0.0094 &     0.1985 &     0.2003 &     0.1952 &     0.1994 &     0.1926 &     0.1926 &     0.1974 &     0.1013 &     0.1908 &     0.2086 &     0.2219 &     0.2039 &     0.2040 \\
solar\_flare\_m0 &     0.0100 &     0.1972 &     0.1999 &     0.1885 &     0.1920 &     0.1917 &     0.1895 &     0.1879 &     0.0965 &     0.2096 &     0.1874 &     0.1872 &     0.1920 &     0.1814 \\
oil &     0.5539 &     0.4606 &     0.4862 &     0.4772 &     0.5097 &     0.4051 &     0.4614 &     0.4647 &     0.4492 &     0.4667 &     0.5277 &     0.5454 &     0.4611 &     0.5142 \\
car\_eval\_4 &     0.8559 &     0.8348 &     0.8479 &     0.8459 &     0.8450 &     0.8067 &     0.8459 &     0.8562 &     0.8348 &     0.8359 &     0.8677 &     0.8665 &     0.8729 &     0.8721 \\
wine\_quality &     0.0043 &     0.1794 &     0.1840 &     0.1769 &     0.1849 &     0.1808 &     0.1787 &     0.1875 &     0.1786 &     0.1784 &     0.1852 &     0.1846 &     0.1806 &     0.1728 \\
letter\_img &     0.7445 &     0.5517 &     0.5913 &     0.5714 &     0.4991 &     0.5595 &     0.5005 &     0.5590 &     0.6423 &     0.5795 &     0.6230 &     0.5148 &     0.6168 &     0.5442 \\
yeast\_me2 &     0.0274 &     0.2646 &     0.2698 &     0.2735 &     0.3084 &     0.2665 &     0.2624 &     0.2875 &     0.3439 &     0.2582 &     0.3115 &     0.3653 &     0.2750 &     0.2946 \\
ozone\_level &     0.0998 &     0.2467 &     0.2603 &     0.2598 &     0.2813 &     0.2218 &     0.2503 &     0.2622 &     0.2426 &     0.2674 &     0.2874 &     0.3058 &     0.2659 &     0.2847 \\
abalone\_19 &     0.0000 &     0.0474 &     0.0487 &     0.0509 &     0.0491 &     0.0432 &     0.0496 &     0.0501 &     0.0450 &     0.0513 &     0.0537 &     0.0527 &     0.0546 &     0.0538 \\ \hline \hline
mean &     0.4297 &     0.4638 &     0.4756 &     0.4733 &     0.4667 &     0.4546 &     0.4530 &     0.4727 &     0.4790 &     0.4738 &     \textcolor{red}{\textbf{0.5033}} &     \textcolor{blue}{\textbf{0.4887}} &     0.4844 &     0.4867 \\
rank &     7.9048 &     9.9762 &     6.9048 &     8.2143 &     7.4286 &     9.5714 &    10.4524 &     7.3810 &     8.2143 &     8.8095 &     \textcolor{red}{\textbf{3.2857}} &     \textcolor{blue}{\textbf{4.7619}} &     6.0000 &     6.0952 \\ \hline

\end{tabular}

}

\end{table*}

==> tables/results_svm_rbf_f1_25.tex <==
\begin{table*}[h!]

\caption{Classification results on benchmark datasets for the SVM classifier with RBF kernel. F1 score averaged over $5$ repeats of $5$-fold (outer) cross-validation is reported. \textcolor{red}{\textbf{Best}} and \textcolor{blue}{\textbf{second-best}} results are highlighted.}
\label{table:svm_rbf_f1}

%\vspace{-0.5em}

\centering

%\renewcommand{\arraystretch}{1.27}

\resizebox{\textwidth}{!}{

\begin{tabular}{l|rrrrrrrrrr|rrrr}
\toprule
 & \fontsize{8}{9}\selectfont\textbf{Imbalanced} & \fontsize{8}{9}\selectfont\textbf{Random} & \fontsize{8}{9}\selectfont\textbf{Global} & \fontsize{8}{9}\selectfont\textbf{SMOTE} & \fontsize{8}{9}\selectfont\textbf{Border.} & \fontsize{8}{9}\selectfont\textbf{Safelevel} & \fontsize{8}{9}\selectfont\textbf{ADASYN} & \fontsize{8}{9}\selectfont\textbf{MWMOTE} & \fontsize{8}{9}\selectfont\textbf{DBSMOTE} & \fontsize{8}{9}\selectfont\textbf{LVQ} & \fontsize{8}{9}\selectfont\textbf{Simplicial} & \fontsize{8}{9}\selectfont\textbf{S-Border.} & \fontsize{8}{9}\selectfont\textbf{S-Safe.} & \fontsize{8}{9}\selectfont\textbf{S-ADASYN} \\  \midrule

ecoli &     0.6238 &     0.6033 &     0.6294 &     0.6284 &     0.6130 &     0.6025 &     0.5989 &     0.6148 &     0.6661 &     0.5995 &     0.6794 &     0.6513 &     0.6390 &     0.6817 \\
optical\_digits &     0.9597 &     0.9741 &     0.9766 &     0.9761 &     0.9691 &     0.9755 &     0.9731 &     0.9749 &     0.9753 &     0.9285 &     0.9752 &     0.9711 &     0.9743 &     0.9740 \\
pen\_digits &     0.9918 &     0.9936 &     0.9916 &     0.9935 &     0.9908 &     0.9938 &     0.9902 &     0.9932 &     0.9925 &     0.9915 &     0.9934 &     0.9905 &     0.9938 &     0.9916 \\
abalone &     0.0000 &     0.3810 &     0.4212 &     0.3883 &     0.3880 &     0.3880 &     0.3783 &     0.3892 &     0.3890 &     0.3583 &     0.4029 &     0.4037 &     0.3948 &     0.3913 \\
sick\_euthyroid &     0.1727 &     0.6027 &     0.6524 &     0.6230 &     0.6069 &     0.5785 &     0.6067 &     0.6175 &     0.6347 &     0.6625 &     0.6614 &     0.6469 &     0.6425 &     0.6486 \\
spectrometer &     0.8474 &     0.8130 &     0.8263 &     0.8205 &     0.8171 &     0.8196 &     0.8211 &     0.8175 &     0.8595 &     0.8582 &     0.8467 &     0.8227 &     0.8419 &     0.8571 \\
car\_eval\_34 &     0.8853 &     0.9372 &     0.9436 &     0.9425 &     0.9411 &     0.8958 &     0.9437 &     0.9457 &     0.9372 &     0.9143 &     0.9414 &     0.9465 &     0.9468 &     0.9450 \\
us\_crime &     0.3589 &     0.5066 &     0.4923 &     0.4818 &     0.5016 &     0.5265 &     0.4657 &     0.4730 &     0.5099 &     0.5412 &     0.4727 &     0.4974 &     0.4611 &     0.4669 \\
yeast\_ml8 &     0.0000 &     0.0319 &     0.0044 &     0.0085 &     0.0065 &     0.0761 &     0.0022 &     0.0000 &     0.0319 &     0.0168 &     0.0000 &     0.0022 &     0.0000 &     0.0000 \\
scene &     0.0175 &     0.2866 &     0.2724 &     0.2674 &     0.2711 &     0.2649 &     0.2655 &     0.2556 &     0.0261 &     0.2090 &     0.2599 &     0.2654 &     0.2199 &     0.2587 \\
libras\_move &     0.8148 &     0.8174 &     0.8030 &     0.8063 &     0.8465 &     0.7280 &     0.8133 &     0.8227 &     0.8174 &     0.7913 &     0.8289 &     0.8271 &     0.8189 &     0.8465 \\
thyroid\_sick &     0.0648 &     0.5457 &     0.5880 &     0.5769 &     0.5717 &     0.4731 &     0.5606 &     0.5754 &     0.5517 &     0.5488 &     0.6443 &     0.6395 &     0.6384 &     0.6459 \\
coil\_2000 &     0.0000 &     0.1934 &     0.1869 &     0.1844 &     0.1845 &     0.1808 &     0.1815 &     0.1814 &     0.0154 &     0.1323 &     0.1773 &     0.1765 &     0.1723 &     0.1761 \\
solar\_flare\_m0 &     0.0000 &     0.1673 &     0.1643 &     0.1614 &     0.1482 &     0.1642 &     0.1625 &     0.1407 &     0.0290 &     0.2409 &     0.1465 &     0.1370 &     0.1384 &     0.1438 \\
oil &     0.3702 &     0.4438 &     0.4752 &     0.4475 &     0.4825 &     0.4193 &     0.4421 &     0.4601 &     0.4447 &     0.4975 &     0.4712 &     0.5242 &     0.4354 &     0.4258 \\
car\_eval\_4 &     0.9677 &     0.9557 &     0.9597 &     0.9583 &     0.9583 &     0.8976 &     0.9583 &     0.9597 &     0.9557 &     0.8887 &     0.9652 &     0.9637 &     0.9624 &     0.9667 \\
wine\_quality &     0.0352 &     0.2425 &     0.1959 &     0.2411 &     0.2538 &     0.2369 &     0.2321 &     0.2128 &     0.1430 &     0.2616 &     0.2408 &     0.2533 &     0.2406 &     0.2365 \\
letter\_img &     0.9522 &     0.9452 &     0.9369 &     0.9559 &     0.9548 &     0.9480 &     0.9569 &     0.9602 &     0.9382 &     0.9521 &     0.9637 &     0.9555 &     0.9626 &     0.9659 \\
yeast\_me2 &     0.0139 &     0.2816 &     0.2872 &     0.2947 &     0.3559 &     0.2672 &     0.2881 &     0.3085 &     0.3485 &     0.3095 &     0.3585 &     0.4163 &     0.3137 &     0.3493 \\
ozone\_level &     0.0000 &     0.3095 &     0.2908 &     0.2956 &     0.3150 &     0.2465 &     0.2955 &     0.3024 &     0.3103 &     0.3489 &     0.3250 &     0.3306 &     0.3169 &     0.3250 \\
abalone\_19 &     0.0000 &     0.0444 &     0.0553 &     0.0503 &     0.0474 &     0.0381 &     0.0500 &     0.0497 &     0.0293 &     0.0484 &     0.0555 &     0.0492 &     0.0613 &     0.0541 \\ \hline 
mean &     0.3846 &     0.5274 &     0.5311 &     0.5287 &     0.5345 &     0.5105 &     0.5232 &     0.5264 &     0.5050 &     0.5286 &     \textcolor{blue}{\textbf{0.5433}} &     \textcolor{red}{\textbf{0.5462}} &     0.5321 &     0.5405 \\
rank &    11.7143 &     7.9524 &     6.3571 &     6.7143 &     7.1429 &     9.1905 &     9.0952 &     7.6905 &     8.1905 &     7.8095 &     \textcolor{red}{\textbf{4.9524}} &     \textcolor{blue}{\textbf{5.6667}} &     6.5238 &     6.0000 \\ \bottomrule

\end{tabular}

}

\end{table*}

==> tables/taxonomy.tex <==
\begin{table}[h!]
\centering

%\vspace{-0.75em}

\caption{Classification of geometric sampling methods.}
%\vspace{0.25em}
\label{table:classification}

\renewcommand{\arraystretch}{1.1}

\begin{tabular}{l|r|r} \hline
                 & \fontsize{9}{10}{\textbf{Neighborhood size}}   & \fontsize{9}{10}{\textbf{Relation arity}} \\ \hline \hline
Random           & $1$                 & $1$                  \\
Global sampling            & $n$                 & $2$                  \\
SMOTE            & $k$                 & $2$                  \\
Simplicial SMOTE & $k$                 & $[3, k]$             \\ \hline
\end{tabular}

\end{table}
